EE-Net: Exploitation-Exploration Neural Networks in Contextual Bandits

In this paper, we propose a novel neural exploration strategy in contextual bandits, EE-Net, distinct from the standard UCB-based and TS-based approaches. Contextual multi-armed bandits have been studied for decades with various applications. To solve the exploitation-exploration tradeoff in bandits, there are three main techniques: epsilon-greedy, Thompson Sampling (TS), and Upper Confidence Bound (UCB). In recent literature, linear contextual bandits have adopted ridge regression to estimate the reward function and combine it with TS or UCB strategies for exploration. However, this line of works explicitly assumes the reward is based on a linear function of arm vectors, which may not be true in real-world datasets. To overcome this challenge, a series of neural bandit algorithms have been proposed, where a neural network is used to learn the underlying reward function and TS or UCB are adapted for exploration. Instead of calculating a large-deviation based statistical bound for exploration like previous methods, we propose "EE-Net", a novel neural-based exploration strategy. In addition to using a neural network (Exploitation network) to learn the reward function, EE-Net uses another neural network (Exploration network) to adaptively learn potential gains compared to the currently estimated reward for exploration. Then, a decision-maker is constructed to combine the outputs from the Exploitation and Exploration networks. We prove that EE-Net can achieve $\mathcal{O}(\sqrt{T\log T})$ regret and show that EE-Net outperforms existing linear and neural contextual bandit baselines on real-world datasets.

==> analysis1.tex <==
%\newpage

\section{Proof of Theorem \ref{theo1}} \label{sec:the1p}

In this section, we provide the proof of Theorem \ref{theo1} and related lemmas.


\proof
For brevity, for the selected arm $\bx_t$ in round $t$, let $h(\bx_t)$ be its expected reward and $ \bx_t^\ast = \arg \max_{i \in [n]} h(\bx_{t,i})$ be the optimal arm in round $t$.

Note that $(\bx_{t,i}, r_{t,i}) \sim \cald$, for each $i \in [n]$. Then, the expected regret of round $t$ is computed by
\iffalse
\begin{equation}
\begin{aligned}
\mathbf{R}_t & = [ r^\ast_t - r_t | \mathbf{X}_t]
& = h(\bx_t^\ast) - h(\bx_t)  \\
&  =  h(\bx_t^\ast)  - f_3(\bx_t)  + f_3(\bx_t) - h(\bx_t) \\
&  \leq \underbrace{  h(\bx_t^\ast) - f_3(\bx_t^\ast) +  f_3(\bx_t)  - f_3(\bx_t)  }_{I_1} +   f_3(\bx_t) - h(\bx_t)  \\
& = h(\bx_t^\ast) - f_3(\bx_t^\ast) + f_3(\bx_t) - h(\bx_t) \\
& \leq  \max_{i \in [n]}  \left( \bbe [ \left(    r_{t, i} -f_3(\bx_{t, i}) \right)  |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} ]  \right) +     \bbe [ \left( f_3(\bx_t)  - r_t \right) |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} ] \\
&  =     \max_{i \in [n]} \left( \bbe \left[  \left(  r_{t, i} - \left(   f_1(\bx_{t, i}; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c \sqrt{mL}; \btheta^2_{t-1}) \right)   \right) \Big |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}   \right]  \right) \\
&  \  \ \    \  \   +     \bbe \left[  \left(   f_1(\bx_t; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1})   - r_t    \right) \Big |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right] \\
& \leq   \max_{i \in [n]} \left( \bbe \left [ | f_1(\bx_{t, i}; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1}) - r_{t, i} | \Big |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right] \right)  \\
&  \  \ \    \  \   +     \bbe \left[  |  f_1(\bx_t; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1})  - r_t  | \Big |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right],
\end{aligned}
\end{equation}
where $I_1$ is because $f_3(\bx_t) = \max_{i \in [n]}f_3(\bx_{t,i})$ and $f_3(\bx_t) - f_3(\bx_t^\ast) \geq 0$.
\fi



\begin{equation}
\begin{aligned}
\mathbf{R}_t 
& =  \underset{(\bx_{t,i}, r_{t,i}),  i \in [n] }{\bbe} [ r^\ast_t - r_t | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}]\\
%& =  \underset{(\bx_{t,i}, r_{t,i}),  i \in [n] }{\bbe} [ r^\ast_t - r_t | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}]\\
& = \bbe_{\bx_{t,i}, i \in [n]} [ h(\bx_t^\ast) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  ]   \\
&  =  \bbe_{\bx_{t,i}, i \in [n]}[h(\bx_t^\ast)  - f_3(\bx_t)  + f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] \\
&  \leq \bbe_{\bx_{t,i}, i \in [n]}[\underbrace{  h(\bx_t^\ast) - f_3(\bx_t^\ast) +  f_3(\bx_t)  - f_3(\bx_t)  }_{I_1} +   f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}]  \\
& =  \bbe_{\bx_{t,i}, i \in [n]}[h(\bx_t^\ast) - f_3(\bx_t^\ast) + f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] \\
& =  \bbe_{\bx_{t,i}, i \in [n]}[h(\bx_t^\ast) - f_3(\bx_t^\ast) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] + \bbe_{\bx_{t,i}, i \in [n]}[f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] \\
& \leq  2 \bbe_{\bx_{t,i}, i \in [n]} \left[  \max_{i \in [n]}  \left(  \left[ \left|   h(\bx_{t, i}) -f_3(\bx_{t, i}) \right|  |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right]  \right) \right]   \\
& =  2 \bbe_{\bx_{t,i}, i \in [n]} \left[  \max_{i \in [n]}  \left(  \left[ \left|  \bbe_{r_{t,i}} [ r_{t,i} | \bx_{t, i} ] -f_3(\bx_{t, i}) \right|  |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right]  \right) \right]   \\
& \overset{(a)}{\leq } 2 \bbe_{\bx_{t,i}, i \in [n]} \left[  \max_{i \in [n]}  \left( \bbe_{r_{t,i}} \left[ \left|   r_{t, i} -f_3(\bx_{t, i}) \right|  |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i} \right]  \right) \right]   \\
& = 2  \bbe_{\bx_{t,i}, i \in [n]} \left[  \max_{i \in [n]} \left( \bbe_{r_{t,i}} \left [\Big | f_1(\bx_{t, i}; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1}) - r_{t, i} \Big| \Big |      \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i}  \right] \right)  \right] \\
& = 2   \bbe_{\bx_{t,i}, i \in [n]} \\
& \ \ \ \  \left[   \max_{i \in [n]} \Bigg( \bbe_{r_{t,i}}
\left[ \Big | f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t,i})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right)  \Big |  \Big |      \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i}  \right] \Bigg) \right]~.
\end{aligned}
\end{equation}
where $I_1$ is because $f_3(\bx_t) = \max_{i \in [n]}f_3(\bx_{t,i})$ and $f_3(\bx_t) - f_3(\bx_t^\ast) \geq 0$, and (a) follows by Jensen's inequality. 

%\ban{Maybe, it is better to remove $\mathbf{X}_t$ in the condition ?}




%\ban{I have a question, if $\bbe[ \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right) | \bx_{t,i}] =  \bbe_{\bx \sim \cald} [ \left(r - f_1(\bx; \btheta_{t-1}^1) \right) ] $ ?}



%\abcomment{If we want to be more rigorous, the above analysis should also be conditioned on the history $(\x_{\tau},r_{\tau}), \tau =1,\ldots,t-1$ because that conditioning shows up below.}

Because, for each $i \in [n]$, $(\bx_{t,i}, r_{t,i}) \sim \cald$, applying Corollary \ref{corollary:main1},
%to $(\bx_{t,i}, r_{t,i}), \forall i \in [n]$,  
with probability at least $(1-\delta)$, we have
\begin{equation}
\mathbf{R}_t  \leq  2 \left(
\sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}}  \right)~.
\end{equation}

Then expected regret of $T$ rounds is computed by
\begin{equation}
\begin{aligned}
\mathbf{R}_T & = \sum_{t =1}^T \mathbf{R}_t\\
 & \leq 2 \sum_{t =1}^T   \left(
\sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}}  \right)  \\
& \leq \underbrace{  (2\sqrt{T} -1) 2\sqrt{2 \epsilon} + 
(2\sqrt{T} -1) 3\sqrt{2}L +  
2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} }_{I_2} \\
&= (2 \sqrt{T} -1 ) ( 2\sqrt{2 \epsilon} + 3\sqrt{2}L) +  2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}
\end{aligned}
\end{equation}
where  $I_2$ is because $\sum_{t=1}^T \frac{1}{\sqrt{t}}  \leq  \int_{1}^T   \frac{1}{\sqrt{t}}  \ dx  +1 =  2 \sqrt{T} -1$ \citep{chlebus2009approximate}.

According to Lemma \ref{lemma:zhu} (1),  with probability at least $1 - \delta$, when $\epsilon \leq  1/T$, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +  (2\sqrt{T} -1) 3\sqrt{2}L +    2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}, 
\end{equation}
As the choice of $m$, we have $\xi \leq \mathcal{O}(1)$. Therefore, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +  (2\sqrt{T} -1) 3\sqrt{2}L  +  \mathcal{O} \left((2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} \right).
\end{equation}
The proof is completed. \qed
%\end{prove*}




\begin{lemma}\label{lemma:main1} [\textbf{Lemma \ref{lemma:main} restated}]
Given $\delta, \epsilon \in (0, 1), \rho \in (0, \mathcal{O}(\frac{1}{L}))$, suppose $m, \eta_1, \eta_2, K_1, K_2$ satisfy the conditions in Eq. (\ref{eq:condi}). Then, with probability at least $1- \delta$, such that it holds for Algorithm \ref{alg:main} that

 \begin{equation}\label{eq:lemmamain}
 \begin{aligned}
 \underset{\substack{(\bx, r) \sim \cald }}{\bbe}  &  \left[ \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right) \right |   |  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right]\\
 & \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(1 /\delta) ) }{t}} ,
 \end{aligned}
 \end{equation}
where $ \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} $ are the data collected up to round $t-1$ and
the expectation is taken over $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.
\end{lemma}





%\abcomment{based on what we choose, the proof below will have to be mildly updated}

\proof 
In this proof, we consider the collected data of up to round $t-1$,  $\{\bx_\tau,  r_\tau \}_{\tau=1}^{t-1}$, as the training dataset and then obtain a generalization bound for it, inspired by \cite{cao2019generalization}.

First, we focus on upper bounding the conditional expectation $\bbe_{r_{t,i}}[ \cdots | \bx_{t,i}]$ in \eqref{eq:lemmamain} with high probability.  For convenience, we use $\bx := \bx_{t,i}, r := r_{t,i}$, noting that the same analysis holds for each $i \in [n]$. Using the Lemma \ref{lemma:gu} (2) and Lemma \ref{lemma:zhu} (2), for any $\tau \in [t-1]$, with probability at least $1 -\delta$, given any $\bx \sim \cald$ and $\| \bx \|_2 \leq 1$,  we have  
%\abcomment{$t$ should be replaced by $\tau = 1,\ldots, t-1$ below, and the subsequent equations ... till we take the expectation over these}
%\abcomment{perhaps state the result for $\widehat{\btheta}^1_t$ since that is what we need later}
\[ \|\triangledown_{\widehat{\btheta}^1_\tau}f(\bx; \widehat{\btheta}^1_\tau)\|_2 \leq \mathcal{O}(\sqrt{mL}). 
\]
Now, consider the exploration network $f_2$.   Given any $\bx \sim \cald$ and $\| \bx \|_2 \leq 1$,  there must exist a constant $c_1$,  such that 
%\abcomment{again, for $\widehat{\btheta}^1_\tau$}
\begin{equation}
\left \| \frac{\triangledown_{\widehat{\btheta}_\tau^1}f_1(\bx; \widehat{\btheta}^1_\tau)}{c_1 \sqrt{mL}}  \right \|_2 \leq  1.
\end{equation}
  Then, applying Lemma \ref{lemma:a},  with probability at least $1-\delta$, for any $t \in [T]$,  we have 

\begin{equation} \label{eq:f2value}
 \left| f_2\left( \frac{\triangledown_{\widehat{\btheta}_\tau^1}f_1( \bx;  \widehat{\btheta}_\tau^1) }{c_1\sqrt{mL} }   ;\widehat{\btheta}_\tau^2\right) \right| \leq  \xi.
\end{equation}

Similarly, applying  Lemma \ref{lemma:a} again,  with probability at least $1-\delta$, for any $t \in [T]$,  we have 
%\abcomment{for $\widehat{\btheta}^1_\tau$} \abcomment{where is $\xi_1$ defined?}
\begin{equation} \label{eq:f1value}
|   f_1(\bx; \widehat{\btheta}_\tau^1 )  | \leq \xi
\end{equation}


Because for any $r \sim \cald$, $|r| \leq 1$, with Eq. (\ref{eq:f2value}) and (\ref{eq:f1value}), 
applying union bound, with probability at least $1 - 2\delta$, we have 
\begin{equation} \label{eq:upperboundoff2}
 \left | f_2 \left( \frac{\triangledown_{ \widehat{ \btheta}_\tau^1 }f_1(\bx; \widehat{ \btheta}_\tau^1)}{c_1\sqrt{mL} }   ; \widehat{\btheta}_\tau^2\right)  -  (r -  f_1(\bx; \widehat{\btheta}_\tau^1 )) \right |  \leq 1  +  2\xi.
\end{equation}

For brevity, let $f_2( \bx ;  \widehat{\btheta}_\tau^2)$ represent $f_2\left( \frac{\triangledown_{\widehat{\btheta}^1_\tau }f_1(\bx ; \widehat{\btheta}_\tau^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_\tau^2\right)$. 


Recall that, for each $\tau \in [t-1]$, 
%\abcomment{we may have used both $\tau \in [t-1]$ and $\tau \in [t]$, pls check}
$\widehat{\btheta}_\tau^1$ and $\widehat{\btheta}_\tau^2$ are the parameters training on $\{\bx_{\tau'}, r_{\tau'} \}_{\tau'=1}^\tau$ according to Algorithm \ref{alg:main}.
Then, we 
define 
\[ V_{\tau} = \bbe_{(\bx, r) \sim D}\left[ \left|f_2( \bx ; \widehat{\btheta}_{\tau-1}^2) - \left(r - f_1(\bx; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right] - \left|f_2( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right) \right|~.
\]

Then, since $(\bx_{\tau},r_{\tau}) \sim \cald$, we have
 \begin{equation} \label{eq:vexp0}
 \begin{aligned}
 \bbe_{(\bx_{\tau}, r_{\tau}) \sim D} [  V_{\tau} | \mathbf{F}_\tau] & =  \bbe_{(\bx, r) \sim D}\left[ \left|f_2\left(  \bx ; \widehat{ \btheta}_{\tau-1}^2\right) - \left(r - f_1(\bx; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \mathbf{F}_\tau \right]  \\
& \quad - \bbe_{(\bx_{\tau}, r_{\tau}) \sim D} \left[  \left|f_2 \left( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right) \right| |  \mathbf{F}_\tau \right] \\
& = 0~,
\end{aligned}
 \end{equation}
where $ \mathbf{F}_\tau$ denotes the $\sigma$-algebra generated by $\{ \bx_{\tau'}, r_{\tau'}\}_{\tau' = 1}^{\tau-1}$. 
%Note that $(\bx_{\tau}, r_{\tau}) \sim D$.

Moreover, we have
\[
\begin{aligned}
\frac{1}{t} \sum_{\tau=1}^t  V_{\tau} & =  \frac{1}{t}  \sum_{\tau=1}^t   \bbe_{(\bx, r) \sim D} \left[ \left|f_2\left( \bx ;   \widehat{\btheta}_{\tau-1}^2\right) 
- \left(r - f_1(\bx; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right]  \\
& \quad - \frac{1}{t}  \sum_{\tau=1}^t \left|f_2\left(\bx_\tau; \widehat{\btheta}_{\tau-1}^2\right) - \left(r_\tau - f_1(\bx_\tau;  \widehat{\btheta}_{\tau-1}^1) \right) \right| .
\end{aligned}
\] 


Since $V_{\tau}$ is a martingale difference sequence, following Lemma 1 in \citep{cesa2004generalization}, applying the Hoeffding-Azuma inequality, 
%to the bounded random variables $V_{1}, \dots, V_{t} $,  
with probability at least $1 - 2\delta$,  we have 
\begin{equation}
\begin{aligned}
    \bbp \left[  \frac{1}{t}  \sum_{\tau=1}^t  V_{\tau}  -   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(\bx, r) \sim D}[ V_{\tau} | \mathbf{F}_{\tau} ] }_{I_1}   >  \underbrace{ ( 1 +  2 \xi)}_{I_2} \sqrt{ \frac{2 \log (1/\delta)}{t}}  \right] &\leq \delta  \\
 \Rightarrow  \qquad  \qquad   \bbp\left[  \frac{1}{t}  \sum_{\tau=1}^t  V_{\tau}   >  ( 1 +  2\xi) \sqrt{ \frac{2 \log (1/\delta)}{t}}  \right] & \leq \delta  ~,
\end{aligned}  
\label{eq:pppuper}
\end{equation}
where $I_1 = 0 $ according to Eq.(\ref{eq:vexp0}) and $I_2$ is because of Eq.(\ref{eq:upperboundoff2}).

According to Algorithm \ref{alg:main}, $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.
Thus, with probability $1 -3\delta$, we have 
\begin{equation}\label{eq:main}
\begin{aligned}
& \underset{\substack{(\bx, r) \sim \cald }}{\bbe}~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| \right] \\
& =     \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(\bx, r) \sim \cald} \left[ \left|f_2 \left( \bx ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r - f_1(\bx; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \right]  \\
& \leq \underbrace{ \frac{1}{t}\sum_{\tau=1}^t \left|f_2 \left( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right)  \right|}_{I_3}   + ( 1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}   ~.
\end{aligned}
\end{equation}

For $I_3$, according to Lemma \ref{lemma:caogeneli},  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$ , we have 
\begin{equation} \label{eq:f12upper}
\begin{aligned}
  & \frac{1}{t}\sum_{\tau=1}^t \left|  f_2 ( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|   \\
   & \leq   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|}_{I_4}  + \frac{3L}{\sqrt{2t}}~.
\end{aligned}
\end{equation}
 For $I_4$, according to  Lemma \ref{lemma:zhu} (1), these exists   $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0  \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, 
such that
\begin{equation} \label{eq:convegene}
\begin{aligned}
 &\frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \\
&\leq  \frac{1}{t} \sqrt{t} \sqrt{ \underbrace{ \sum_{\tau=1}^t \left(   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2}_{I_5} } \\
&\leq  \frac{1}{\sqrt{t}}\sqrt{ \underbrace{2\epsilon}_{I_5}}~, 
\end{aligned}
\end{equation}
where $I_5$ follows by a direct application of  Lemma \ref{lemma:zhu} (1) by defining the loss $\mathcal{L}(\widetilde{\btheta}^2) =\frac{1}{2}\sum_{\tau=1}^t \left(   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2 \leq \epsilon$. 

Combining Eq.(\ref{eq:main}), Eq.(\ref{eq:f12upper}) and Eq.(\ref{eq:convegene}), with probability $(1-3\delta)$ we have 
%\abcomment{need to mention expectation over $\btheta^1,\btheta^2$}
\begin{equation}\label{eq:fincon}
\begin{aligned}
 & \bbe_{(\bx, r) \sim \cald}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| | \{ \bx_{\tau}, r_{\tau}\}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~.
 \end{aligned}
\end{equation}
where the expectation over $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.

Then, applying union bound and rescaling the $\delta$ complete the proof. \qed







\begin{corollary}\label{corollary:main1} 
Given $\delta, \epsilon \in (0, 1), \rho \in (0, \mathcal{O}(\frac{1}{L}))$, suppose $m, \eta_1, \eta_2, K_1, K_2$ satisfy the conditions in Eq. (\ref{eq:condi}). Then, with probability at least $1- \delta$,  for any round $\tau \in [t], i \in [n]$, there exists a constant $c_1 > 0$, such that it holds uniformly for Algorithm \ref{alg:main} that
\begin{equation}\label{eq:lemmamain}
\begin{aligned}
\underset{\bx_{t,i}, i \in [n]}{\bbe} \bigg[ \max_{i \in [n]} \Bigg( \underset{r_{t,i}}{\bbe}   &  \bigg[ \Big | f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t,i}; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right) \Big |   \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i}  \bigg] \Bigg) \Bigg]\\
& \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}} ,
\end{aligned}
\end{equation}
where $ \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} $ are the data collected up to round $t-1$ and
the expectation is taken over $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.
\end{corollary}

\proof
This a direct corollary of Lemma \ref{lemma:main1}.
According to Eq. (\ref{eq:fincon}),
with probability $1-3\delta$,  given $ (\bx, r) \sim \cald$, we have 
%\abcomment{need to mention expectation over $\btheta^1,\btheta^2$}
\begin{equation}
\begin{aligned}
 & \underset{ \bx }{\bbe}  ~ \underset{r}{\bbe}     ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right|  \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~.
 \end{aligned}
\end{equation}


Then, in round $t$,  applying the union bound, for $(\bx_{t,i}, r_{t,i}) \sim \cald, \forall i \in [n]$,  with probability $1 - 3n \delta$, we have

\begin{equation}
\begin{aligned}
\forall i \in [n],  \ \  & \underset{\bx_{t,i}}{\bbe}  ~ \underset{r_{r,i}}{\bbe}     ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx_{t, i} ; \btheta_{t-1}^2\right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right)  \right|  \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~,
 \end{aligned}
\end{equation}

which is equal to
\begin{equation}
\begin{aligned}
\underset{\bx_{t,i}, i \in [n]}{\bbe} \bigg[ \max_{i \in [n]} \bigg( \underset{r_{t,i}}{\bbe}~ \underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}  &  \left[ \left|f_2 \left( \bx_{t,i} ; \btheta_{t-1}^2\right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right)  \right|   \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i}  \right]  \bigg) \bigg]\\
& \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log (1 /\delta) }{t}}.
 \end{aligned}
\end{equation}
Then, apply union bound for any round $\tau \in [t]$, to help the proof for Theorem \ref{theo1}. Rescaling the $\delta$ and replacing $f_2$ with the formal form complete the proof.


\iffalse
Note that the same analysis can be done conditioned on $\bx := \bx_{t,i}$ such that 
\begin{equation*}
%\label{eq:fincon2}
\begin{aligned}
\bbp \left( \bbe_{r_{t,i} } ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| \mid \bx_{t,i} \right] \right. \geq  \left. \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta') }{t}} \right) \leq 3\delta'~.
 \end{aligned}
\end{equation*}
Since $\bx_{t,i}, i \in [n]$ are drawn i.i.d.,~ by union bound and using $\delta = t n \delta'$, with probability $(1-\delta)$ we have
\begin{equation*}
%\label{eq:fincon2}
\begin{aligned}
\max_{i \in [n]} \left( \bbe_{r_{t,i} } ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| \mid \bx_{t,i} \right] \right) \leq  \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (t n/\delta) }{t}} ~.
 \end{aligned}
\end{equation*}
Taking expectation w.r.t.~$\bx_{t,i}, i\in [n]$ completes the proof. 
\fi
\qed


%\abcomment{Have not explained why we need to take union bound over $t$, will be good to add that. Note that we have not maintianed the conditioning w.r.t.~the history $F_{\tau}$ through the proof, will also be good to do that.}












\begin{lemma} \label{lemma:a}
 
 Let $f(\cdot; \widehat{\btheta}_t)$ follow the stochastic gradient descent of $f_1$ or $f_2$ in Algorithm \ref{alg:main}.
 Suppose $m, \eta_1, \eta_2$ satisfy the conditions in Eq. (\ref{eq:condi}).  With probability at least $1 - \delta$, for any $\bx$ with $\|\bx\|_2 = 1$ and $t \in [T]$, it holds that
\[
| f(\bx; \widehat{\btheta}_t)| \leq  \mathcal{O}(1) +  \mathcal{O} \left( \frac{t^3n L \log m}{ \rho \sqrt{m} } \right) + \mathcal{O} \left(  \frac{t^4 n L^2  \log^{11/6} m}{ \rho  m^{1/6}}\right).
\]
\end{lemma}



%\begin{prove*}
\proof Considering an inequality $ |a - b| \leq c$, we have $|a| \leq |b| + c$. 
Let $\btheta_0$ be randomly initialized. Then applying  Lemma \ref{lemma:gu} (1),  for any $\bx \sim \mathcal{D}, \|\bx \|_2 = 1$ and $ \|\widehat{\btheta}_t - \btheta_0\| \leq w$,  we have 
\begin{equation}
\begin{aligned}
|f(\bx; \widehat{\btheta}_t) | &\leq  | f(\bx; \btheta_0)| +  |\langle  \triangledown_{\btheta_0}f(\bx_i; \btheta_0), \widehat{\btheta}_t - \btheta_0   \rangle  | +   \mathcal{O} ( L^2 \sqrt{m \log(m)}) \|\widehat{\btheta}_t - \btheta_0 \|_2 w^{1/3} \\
&  \leq \underbrace{\mathcal{O}(1)}_{I_0}  +  \underbrace{  \|  \triangledown_{\btheta_0}f(\bx_i; \btheta_0)  \|_2 \| \widehat{\btheta}_t - \btheta_0  \|_2}_{I_1}  + \mathcal{O} ( L^2 \sqrt{m \log(m)}) \|\widehat{\btheta}_t - \btheta_0 \|_2 w^{1/3} \\
& \leq \mathcal{O}(1) +  \underbrace{  \mathcal{O} (L) \cdot  \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)}_{I_2} + \underbrace{   \mathcal{O} \left( L^2 \sqrt{m \log(m)} \right) \cdot  \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)^{4/3} }_{I_3}  \\
&  =  \mathcal{O}(1) +  \mathcal{O} \left( \frac{t^3 L \log m}{ \rho \sqrt{m} } \right) + \mathcal{O} \left(  \frac{t^4 L^2  \log^{11/6} m}{ \rho  m^{1/6}}\right)
\end{aligned}
\end{equation}
where: $I_0$ is based on the Lemma \ref{lemma:zhu} (3);
$I_1$ is an application of Cauchy–Schwarz inequality; $I_2$ is according to  Lemma \ref{lemma:zhu} (2) and (3) in which $\widehat{\btheta}_t$ can be considered as one step gradient descent; $I_3$ is due to Lemma \ref{lemma:zhu} (2).

Then, the proof is completed. \qed
%\end{prove*}












\begin{lemma} \label{lemma:zhu}
Given a constant $0 < \epsilon < 1$, suppose $m \geq  \widetilde{\Omega}   \left ( \text{poly}(T, n, L, \rho^{-1}) \cdot    e^{\sqrt{\log 1/\delta }}  \right ) $, the learning rate $\eta = \Omega(\frac{\rho}{ \text{poly} (t ,n, L) m} ) $, the number of iterations $K = \Omega (\frac{\text{poly}(t, n, L)}{\rho^2} \cdot \log \epsilon^{-1})$. Then, with probability at least $1 - \delta$,  starting from random initialization $\btheta_0$, 
\begin{enumerate}[label=(\arabic*)]
    \item (Theorem 1 in \citep{allen2019convergence}) 
    In round $t \in [T]$, given the collected data $\{\bx_\tau, r_\tau\}_{i=\tau}^{t}$, the loss function is defined as:
    $\mathcal{L}(\btheta) = \frac{1}{2} \sum_{\tau = 1}^{t}   \left( f(\bx_{\tau}; \btheta) - r_\tau \right)^2$.
    Then,  there exists  $\widetilde{\btheta}$  satisfying $\|\widetilde{\btheta} - \btheta_0\|_2 \leq \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)$, such that
    $ \mathcal{L}(\widetilde{\btheta}) \leq \epsilon $ in $K = \Omega (\frac{\text{poly}(t, n, L)}{\rho^2} \cdot \log \epsilon^{-1})$ iterations;\\
    \item (Theorem 1 in \citep{allen2019convergence}) For any $k \in [K]$, it holds uniformly that
    $
    \|\btheta^{(k)}_t - \btheta_0\|_2 \leq \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)
    $;
    \item Following the initialization, it holds that
    \[
     \|   \triangledown_{\btheta_0 }f(\bx_i; \btheta_0)  \|_2 \leq \mathcal{O} (L),   \    \   \
      |  f(\bx_i; \btheta_0)  | \leq \mathcal{O} (1)
    \]
\end{enumerate}
where $\btheta^{(k)}_t$ represents the parameters of $f$ after $k \in [K] $ iterations if gradient descent in round $t$.
\end{lemma}

%\begin{prove*}
\proof 
Note that the output dimension $d$ in \citep{allen2019convergence} is removed because the output of network function in this paper always is a scalar.
For (1) and (2),  the only different setting from \citep{allen2019convergence} is that the initialization of last layer $\bw_{L} \sim \mathcal{N}(0, \frac{2}{m})$ in this paper while $\bw_{L} \sim \mathcal{N}(0, \frac{1}{d})$ in \citep{allen2019convergence}. Because $d =1$ and $m > d$ here, the upper bound in \citep{allen2019convergence} still holds for $\bw_L$: with probability at least $1 - \exp{(- \Omega(m/L))}, \|\bw_L\|_F \leq \sqrt{m/d}$. Therefore, it is easy to verify that (1) and (2) still hold for the initialization of this paper.

For (3), based on Lemma 7.1 in \cite{allen2019convergence}, we have $ |  f(\bx_i; \btheta_0)  | \leq \mathcal{O} (1)$. Denote by $D$ the ReLU function.  For any $l \in [L]$, 
\[
\|\triangledown_{W_l}f(\bx_i; \btheta_0)\|_F \leq   \|\bw_L D \bw_{L-1} \cdots D \bw_{l+1}\|_F \cdot \| D \bw_{l+1} \cdots \bx \|_F \leq  \mathcal{O}(\sqrt{L}) 
\] 
where the inequality is according to Lemma 7.2 in \cite{allen2019convergence}. Therefore, we have $ \|   \triangledown_{\btheta_0 }f(\bx_i; \btheta_0)  \|_2 \leq \mathcal{O} (L) $. \qed 
%\end{prove*}




\begin{lemma} [Lemma 4.1, \citep{cao2019generalization}]  \label{lemma:gu} 
Suppose $ \mathcal{O}( m^{-3/2} L^{-3/2} [ \log (TnL^2/\delta) ]^{3/2}  )   \leq w \leq  \mathcal{O} (L^{-6}[\log m]^{-3/2} )$. Then,
with probability at least $1- \delta$ over randomness of $\btheta_0$, for any $ t \in [T], \|\bx \|_2 =1 $, and $\btheta, \btheta'$
satisfying $\| \btheta - \btheta_0 \|_2 \leq w$ and $\| \btheta' - \btheta_0 \|_2 \leq w$
, it holds uniformly that
\begin{enumerate}[label=(\arabic*)]
 \item $
| f(\bx_i; \btheta) - f(\bx_i; \btheta') -  \langle  \triangledown_{\btheta'}f(\bx_i; \btheta'), \btheta - \btheta'    \rangle    | \leq \mathcal{O} (w^{1/3}L^2 \sqrt{m \log(m)}) \|\btheta - \btheta'\|_2
$
\item $  \| \triangledown_{\btheta}f(\bx; \btheta)\|_2  \leq \mathcal{O}(\sqrt{mL})$.
\end{enumerate}
\end{lemma}


\begin{lemma} \label{lemma:caogeneli}
For any $\delta > 0$, suppose
\[
m > \tilde{\mathcal{O}}\left(  \text{poly} (T, n, \rho^{-1}, L, \log (1/\delta) \cdot e^{\sqrt{ \log 1/\delta}}) \right), \ \ \nu = \tilde{\Theta}(t^6/\delta^2).  
\]
Then, with probability at least $1 - \delta$, setting $\eta_2 = \Theta( \frac{ \nu}{\sqrt{2} t m})$ for algorithm \ref{alg:main},   for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$  such that
\[
\begin{aligned}
\sum_{\tau=1}^t \left|   f_2 \left( \frac{\triangledown_{\widehat{\btheta}_{\tau-1}^1 }f_1(\bx_\tau ; \widehat{\btheta}_{\tau-1}^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_{\tau-1}^2  \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| \\
\leq   \sum_{\tau=1}^t \left|   f_2  \left( \frac{\triangledown_{\widehat{\btheta}_{\tau-1}^1}f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_{t}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| + \frac{3L\sqrt{t} }{\sqrt{2}}\\
\end{aligned}
\]
\end{lemma}
\begin{proof}
This is a direct application of Lemma 4.3 in \citep{cao2019generalization} by setting $R = \frac{t^3}{\rho} \log m,  \epsilon = \frac{LR}{ \sqrt{2\nu t}}$,  and $ \nu = R^2$.
We set $L_\tau( \widehat{\btheta}_{\tau -1}^2 ) =  \left |  f_2 ( \triangledown_{\widehat{\btheta}_{\tau-1}^1} f_1  ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| $.
Based on Lemma \ref{lemma:zhu} (2), for any $\tau \in [t]$, we have 
\[ 
\|\widehat{\btheta}_{\tau}^2 - \widehat{\btheta}_{\tau-1}^2\|_2 \leq  \| \widehat{\btheta}_{\tau}^2 - \btheta_0 \|_2 + \| \btheta_0 -   \widehat{\btheta}_{\tau-1}^2 \|_2 \leq \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m).
\]
Then, according to Lemma 4.3 in \citep{cao2019generalization}, then,  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, we have 
\begin{equation}
\sum_{\tau=1}^t  L_\tau( \widehat{\btheta}_{\tau -1}^2 ) \leq \sum_{\tau=1}^t L_\tau( \widetilde{\btheta}^2) + 3 t \epsilon.
\end{equation}
Then, replacing $\epsilon$ completes the proof.
\end{proof}







==> analysis1_new.tex <==
%\newpage

\section{Proof of Theorem \ref{theo1}} \label{sec:the1p}

In this section, we provide the proof of Theorem \ref{theo1} and related lemmas.


\proof
For brevity, for the selected arm $\bx_t$ in round $t$, let $h(\bx_t)$ be its expected reward and $ \bx_t^\ast = \arg \max_{i \in [n]} h(\bx_{t,i})$ be the optimal arm in round $t$.
%
Note that $(\bx_{t,i}, r_{t,i}) \sim \cald$, for each $i \in [n]$. Since $p(\bx_{t,i},r_{t,i}) = p(\bx_{t,i}) p(r_{t,i}|\bx_{t,i})$, we denote the marginal distribution of $\bx_{t,i}$ as $\cald_{\bx}$ and the conditional distribution of $r_{t,i}$ as $\cald_{r|\bx_{t,i}}$ so that $\bx_{t,i} \sim \cald_{\bx}$ and $r_{t,i} \sim \cald_{r|\bx_{t,i}}$. Let $X_t = \{ \bx_{t,i}, i \in [n]\}$ and note that $\bbe_{r_{t,i} \sim \cald_{r|X_t}}[r_{t,i}] = h(\bx_{t,i})$.

% \iffalse
% \begin{equation}
% \begin{aligned}
% \mathbf{R}_t 
% %& = [ r^\ast_t - r_t | \mathbf{X}_t]
% & = h(\bx_t^\ast) - h(\bx_t)  \\
% &  =  h(\bx_t^\ast)  - f_3(\bx_t)  + f_3(\bx_t) - h(\bx_t) \\
% &  \leq \underbrace{  h(\bx_t^\ast) - f_3(\bx_t^\ast) +  f_3(\bx_t)  - f_3(\bx_t)  }_{I_1} +   f_3(\bx_t) - h(\bx_t)  \\
% & = h(\bx_t^\ast) - f_3(\bx_t^\ast) + f_3(\bx_t) - h(\bx_t) \\
% & \leq  \max_{i \in [n]}  \left( \bbe [ \left(    r_{t, i} -f_3(\bx_{t, i}) \right)  |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} ]  \right) +     \bbe [ \left( f_3(\bx_t)  - r_t \right) |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} ] \\
% &  =     \max_{i \in [n]} \left( \bbe \left[  \left(  r_{t, i} - \left(   f_1(\bx_{t, i}; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c \sqrt{mL}; \btheta^2_{t-1}) \right)   \right) \Big |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}   \right]  \right) \\
% &  \  \ \    \  \   +     \bbe \left[  \left(   f_1(\bx_t; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1})   - r_t    \right) \Big |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right] \\
% & \leq   \max_{i \in [n]} \left( \bbe \left [ | f_1(\bx_{t, i}; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1}) - r_{t, i} | \Big |     \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right] \right)  \\
% &  \  \ \    \  \   +     \bbe \left[  |  f_1(\bx_t; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1})  - r_t  | \Big |    \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  \right],
% \end{aligned}
% \end{equation}
% where $I_1$ is because $f_3(\bx_t) = \max_{i \in [n]}f_3(\bx_{t,i})$ and $f_3(\bx_t) - f_3(\bx_t^\ast) \geq 0$.
% \fi


Now, the expected regret of round $t$ is given by
\begin{equation}
\begin{aligned}
\mathbf{R}_t 
& =  h(\bx_t^\ast) - h(\bx_t)    \\
&  =  h(\bx_t^\ast)  - f_3(\bx_t)  + f_3(\bx_t) - h(\bx_t) \\
&  \leq \underbrace{  h(\bx_t^\ast) - f_3(\bx_t^\ast) +  f_3(\bx_t)  - f_3(\bx_t)  }_{I_1} +   f_3(\bx_t) - h(\bx_t)  \\
& =  h(\bx_t^\ast) - f_3(\bx_t^\ast) + f_3(\bx_t) - h(\bx_t)  \\
& \leq  2   \max_{i \in [n]}   \left|   h(\bx_{t, i}) -f_3(\bx_{t, i}) \right|    \\
& =  2   \max_{i \in [n]}   \left|  \bbe_{r_{t,i} \sim \cald_{r|X_t}} [ r_{t,i} ] -f_3(\bx_{t, i}) \right|       \\
& \overset{(a)}{\leq } 2  \max_{i \in [n]}   \bbe_{r_{t,i} \sim \cald_{r|X_t}} \left|   r_{t, i} -f_3(\bx_{t, i}) \right|   \\
& = 2    \max_{i \in [n]} \bbe_{(\btheta^1_{t-1},\btheta^2_{t-1})} \bbe_{r_{t,i} \sim \cald_{r|X_t}} \Big | f_1(\bx_{t, i}; \btheta^1_{t-1}) + f_2(\triangledown_{\btheta^1_{t-1}}f_1/c\sqrt{mL}; \btheta^2_{t-1}) - r_{t, i} \Big |  \\
& = 2     \max_{i \in [n]} \bbe_{(\btheta^1_{t-1},\btheta^2_{t-1})} \bbe_{r_{t,i} \sim \cald_{r|X_t}} \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t,i})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right)  \right|  ~.
\end{aligned}
\end{equation}
where $I_1$ is because $f_3(\bx_t) = \max_{i \in [n]}f_3(\bx_{t,i})$ and $f_3(\bx_t) - f_3(\bx_t^\ast) \geq 0$, and (a) follows by Jensen's inequality. 

%\ban{Maybe, it is better to remove $\mathbf{X}_t$ in the condition ?}

%\ban{I have a question, if $\bbe[ \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right) | \bx_{t,i}] =  \bbe_{\bx \sim \cald} [ \left(r - f_1(\bx; \btheta_{t-1}^1) \right) ] $ ?}

%\abcomment{If we want to be more rigorous, the above analysis should also be conditioned on the history $(\x_{\tau},r_{\tau}), \tau =1,\ldots,t-1$ because that conditioning shows up below.}

%Because, for each $i \in [n]$, $(\bx_{t,i}, r_{t,i}) \sim \cald$, 

Applying Corollary \ref{corollary:main1}, with probability at least $(1-3\delta)$, we have
\begin{equation}
\mathbf{R}_t  \leq  2 \left(
\sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}}  \right)~.
\end{equation}

Then expected regret of $T$ rounds is computed by
\begin{equation}
\begin{aligned}
\mathbf{R}_T & = \sum_{t =1}^T \mathbf{R}_t\\
 & \leq 2 \sum_{t =1}^T   \left(
\sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}}  \right)  \\
& \leq \underbrace{  (2\sqrt{T} -1) 2\sqrt{2 \epsilon} + 
(2\sqrt{T} -1) 3\sqrt{2}L +  
2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} }_{I_2} \\
&= (2 \sqrt{T} -1 ) ( 2\sqrt{2 \epsilon} + 3\sqrt{2}L) +  2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}
\end{aligned}
\end{equation}
where  $I_2$ is because $\sum_{t=1}^T \frac{1}{\sqrt{t}}  \leq  \int_{1}^T   \frac{1}{\sqrt{t}}  \ dx  +1 =  2 \sqrt{T} -1$ \citep{chlebus2009approximate}.

According to Lemma \ref{lemma:zhu} (1),  with probability at least $1 - \delta$, when $\epsilon \leq  1/T$, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +  (2\sqrt{T} -1) 3\sqrt{2}L +    2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}, 
\end{equation}
As the choice of $m$, we have $\xi \leq \mathcal{O}(1)$. Therefore, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +  (2\sqrt{T} -1) 3\sqrt{2}L  +  \mathcal{O} \left((2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} \right).
\end{equation}
The proof is completed. \qed
%\end{prove*}




\begin{lemma}\label{lemma:main1} [\textbf{Lemma \ref{lemma:main} restated}]
Given $\delta, \epsilon \in (0, 1), \rho \in (0, \mathcal{O}(\frac{1}{L}))$, suppose $m, \eta_1, \eta_2, K_1, K_2$ satisfy the conditions in (\ref{eq:condi}). Then, with probability at least $(1- 3\delta)$ over the random initialization and the draws of $\bx_{\tau,i} \sim \cald_{\bx}, i \in [n], \tau \in [t-1]$, with $X_t = \{\bx_{t,i}, i \in [n]\}$, it holds that
 \begin{equation}\label{eq:lemmamain}
 \begin{aligned}
\bbe_{(\btheta^1_{t-1},\btheta^2_{t-1})} \bbe_{r_{t,i} \sim \cald_{r|X_t}}  &  \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t,i}; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right) \right |  \\
 & \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(1 /\delta) ) }{t}} ,
 \end{aligned}
 \end{equation}
where $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ are  uniformly drawn from $(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2), \tau \in [t-1]$, the parameters estimated in Algorithm \ref{alg:main} using historical data $(\bx_{\tau},r_{\tau}), \tau \in [t-1]$.
\end{lemma}





%\abcomment{based on what we choose, the proof below will have to be mildly updated}

\proof 
In this proof, we consider the collected data of up to round $t-1$,  $\{\bx_\tau,  r_\tau \}_{\tau=1}^{t-1}$, as the training dataset and then obtain a generalization bound for it, inspired by \cite{cao2019generalization}.

For convenience, let $\bx := \bx_{\tau,i}, r := r_{\tau,i}$, noting that the same analysis holds for each $i \in [n], \tau \in [t-1]$. Using the Lemma \ref{lemma:gu} (2) and Lemma \ref{lemma:zhu} (2), for any $\tau \in [t-1]$ and any $\bx \sim \cald_{\bx}$ with $\| \bx \|_2 \leq 1$, with probability at least $(1 -\delta)$ over the random initialization,   we have  
\[ \|\triangledown_{\widehat{\btheta}^1_\tau}f(\bx; \widehat{\btheta}^1_\tau)\|_2 \leq \mathcal{O}(\sqrt{mL}). 
\]
Now, consider the exploration network $f_2$.   Given any $\bx \sim \cald$ and $\| \bx \|_2 \leq 1$,  there must exist a constant $c_1$,  such that 
%\abcomment{again, for $\widehat{\btheta}^1_\tau$}
\begin{equation}
\left \| \frac{\triangledown_{\widehat{\btheta}_\tau^1}f_1(\bx; \widehat{\btheta}^1_\tau)}{c_1 \sqrt{mL}}  \right \|_2 \leq  1.
\end{equation}
Then, applying Lemma \ref{lemma:a},  with probability at least $(1-\delta)$ over the initialization,  we have 
\begin{equation} \label{eq:f2value}
 \left| f_2\left( \frac{\triangledown_{\widehat{\btheta}_\tau^1}f_1( \bx;  \widehat{\btheta}_\tau^1) }{c_1\sqrt{mL} }   ;\widehat{\btheta}_\tau^2\right) \right| \leq  \xi.
\end{equation}
\abcomment{will be good to refer to the statement/equation which defines $\xi$}

Similarly, applying  Lemma \ref{lemma:a} again,  with probability at least $(1-\delta)$ over the initialization, we have 
%\abcomment{for $\widehat{\btheta}^1_\tau$} \abcomment{where is $\xi_1$ defined?}
\begin{equation} \label{eq:f1value}
|   f_1(\bx; \widehat{\btheta}_\tau^1 )  | \leq \xi  ~.
\end{equation}

Because for any $r \sim \cald_{r|\bx}$, $|r| \leq 1$, from \eqref{eq:f2value} and \eqref{eq:f1value}, applying union bound we get: with probability at least $(1 - 2\delta)$ over the random initialization, we have 
\begin{equation} \label{eq:upperboundoff2}
 \left | f_2 \left( \frac{\triangledown_{ \widehat{ \btheta}_\tau^1 }f_1(\bx; \widehat{ \btheta}_\tau^1)}{c_1\sqrt{mL} }   ; \widehat{\btheta}_\tau^2\right)  -  (r -  f_1(\bx; \widehat{\btheta}_\tau^1 )) \right |  \leq 1  +  2\xi.
\end{equation}
Noting that \eqref{eq:upperboundoff2} is for $\bx = \bx_{t,i}$ for a specific $t \in [T], i \in [n]$, by union bound, \eqref{eq:upperboundoff2} holds $\forall t \in [T], i \in [n]$ with probability at least $(1-nT \delta)$. For brevity, we will use 
$f_2( \bx ;  \widehat{\btheta}_\tau^2) := f_2\left( \triangledown_{\widehat{\btheta}^1_\tau }f_1(\bx ; \widehat{\btheta}_\tau^1)/(c_1\sqrt{mL}) ; \widehat{\btheta}_\tau^2\right)$ in the sequel.


Define $i_{\tau} := \text{argmax}_{i \in [n]}~f_1(\bx_{\tau,i}; \widehat{ \btheta}_\tau^1) + f_2( \bx_{\tau,i} ;  \widehat{\btheta}_\tau^2)$. Given $X_{\tau} = \{ \bx_{\tau,i}, i \in [n]\}$, note that $i_{\tau}$ is fixed. For $r_{t,i} \sim \cald_{r|X_t}$ for $i \in [n]$, $r_{\tau,i_{\tau}}$ is the random reward drawn corresponding to the pre-fixed index $i_{\tau}$.

Define
\begin{align*}
V_{\tau} & := \bbe_{r'_{\tau,i_{\tau}} \sim \cald_{r|X_t}} \left[ \left|f_2( \bx_{\tau,i_{\tau}} ; \widehat{\btheta}_{\tau-1}^2) - \left(r'_{\tau,i_{\tau}} 
 - f_1(\bx_{\tau,i_{\tau}}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right] \\
& \qquad \qquad - \left|f_2( \bx_{\tau,i_{\tau}} ; \widehat{\btheta}_{\tau-1}^2) - \left(r_{\tau,i_{\tau}} - f_1(\bx_{\tau,i_{\tau}}; \widehat{\btheta}_{\tau-1}^1) \right) \right|~,
\end{align*}
where for each $\tau \in [t-1]$, 
$\widehat{\btheta}_\tau^1$ and $\widehat{\btheta}_\tau^2$ are the parameters training on $\{\bx_{\tau'}, r_{\tau'} \}_{\tau'=1}^\tau$ according to Algorithm \ref{alg:main}.
%\abcomment{$V_{\tau}$ should be based on $(\bx_{\tau, i_{\tau}}, r_{\tau, i_{\tau}})$ where $i_{\tau}$ is a function of $\bx_{\tau,i}, i \in [n]$, and the analysis should be conditioned on this. Lets check if this works, and if the analysis can be done conditioned on $\bx_{\tau,i}, i \in [n]$.}

%Then, since $(\bx_{\tau,i},r_{\tau,i}) \sim \cald$, 
Then, with $\mathbf{F}_{\tau}$ denoting the $\sigma$-algebra corresponding to $({\cal H}_{t-1}, X_t)$ where the history ${\cal H}_{\tau-1} = \{ \bx_{\tau'}, r_{\tau'}\}_{\tau' = 1}^{\tau-1}$,
we have 
\begin{equation} \label{eq:vexp0}
\begin{aligned}
\bbe_{r_{\tau,i_{\tau}} \sim \cald_{r|X_{\tau}}} [  V_{\tau} | \mathbf{F}_{\tau}] 
& =  \bbe_{r'_{\tau,i_{\tau}} \sim \cald_{r|X_t}} \left[ \left|f_2\left(  \bx_{\tau,i_{\tau}} ; \widehat{ \btheta}_{\tau-1}^2\right) - \left(r'_{\tau,i_{\tau}} - f_1(\bx_{\tau,i_{\tau}}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \bigg| \mathbf{F}_{\tau} \right]  \\
& \qquad - \bbe_{r_{\tau,i_{\tau}} \sim \cald_{r|X_{\tau}}} \left[  \left|f_2 \left( \bx_{\tau,i_{\tau}} ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_{\tau,i_\tau} - f_1(\bx_{\tau,i_{\tau}}; \widehat{\btheta}_{\tau-1}^1) \right) \right| \bigg|  \mathbf{F}_{\tau} \right] \\
& \overset{(a)}{=} 0~,
\end{aligned}
 \end{equation}
where (a) follows since $i_{\tau}$ is a constant (measurable) conditioned on $X_{\tau}$, so that $r_{\tau,i_{\tau}}$ conditioned on $X_t$ is identically distributed as $r_{\tau,i}$ for any $i \in [n]$. In other words, since the index $i_{\tau}$ is getting fixed ahead of time conditioned on $X_{\tau}$ and before the $r_{\tau,i}, i \in [n]$ are drawn, $r_{\tau,i_{\tau}}$ has the same distribution as $r_{t,i}$ for any $i \in [n]$. 

\abcomment{Stopping here, because this analysis will not work. In particular, we need an analysis for a general $i \in [n]$ and the above argument will only yield an analysis for $i_{\tau}$ but not $i \neq i_{\tau}$.}

Moreover, we have
\[
\begin{aligned}
\frac{1}{t} \sum_{\tau=1}^t  V_{\tau} & =  \frac{1}{t}  \sum_{\tau=1}^t   \bbe_{(\bx, r) \sim D} \left[ \left|f_2\left( \bx ;   \widehat{\btheta}_{\tau-1}^2\right) 
- \left(r - f_1(\bx; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right]  \\
& \quad - \frac{1}{t}  \sum_{\tau=1}^t \left|f_2\left(\bx_{\tau,i}; \widehat{\btheta}_{\tau-1}^2\right) - \left(r_{\tau,i} - f_1(\bx_{\tau,i};  \widehat{\btheta}_{\tau-1}^1) \right) \right| .
\end{aligned}
\] 


Since $V_{\tau}$ is a martingale difference sequence, following Lemma 1 in \citep{cesa2004generalization}, applying the Hoeffding-Azuma inequality, 
%to the bounded random variables $V_{1}, \dots, V_{t} $,  
with probability at least $1 - 2\delta$,  we have 
\begin{equation}
\begin{aligned}
    \bbp \left[  \frac{1}{t}  \sum_{\tau=1}^t  V_{\tau}  -   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(\bx, r) \sim D}[ V_{\tau} | \mathbf{F}_{\tau} ] }_{I_1}   >  \underbrace{ ( 1 +  2 \xi)}_{I_2} \sqrt{ \frac{2 \log (1/\delta)}{t}}  \right] &\leq \delta  \\
 \Rightarrow  \qquad  \qquad   \bbp\left[  \frac{1}{t}  \sum_{\tau=1}^t  V_{\tau}   >  ( 1 +  2\xi) \sqrt{ \frac{2 \log (1/\delta)}{t}}  \right] & \leq \delta  ~,
\end{aligned}  
\label{eq:pppuper}
\end{equation}
where $I_1 = 0 $ according to Eq.(\ref{eq:vexp0}) and $I_2$ is because of Eq.(\ref{eq:upperboundoff2}).

According to Algorithm \ref{alg:main}, $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.
Thus, with probability $1 -3\delta$, we have 
\begin{equation}\label{eq:main}
\begin{aligned}
& \underset{\substack{(\bx, r) \sim \cald }}{\bbe}~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| \right] \\
& =     \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(\bx, r) \sim \cald} \left[ \left|f_2 \left( \bx ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r - f_1(\bx; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \right]  \\
& \leq \underbrace{ \frac{1}{t}\sum_{\tau=1}^t \left|f_2 \left( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right)  \right|}_{I_3}   + ( 1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}   ~.
\end{aligned}
\end{equation}
\ban{ 
Here, will change to 
\[
\begin{aligned}
& \underset{\substack{(r_t) \sim \cald }}{\bbe}~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx_t ; \btheta_{t-1}^2\right) - \left(r_t - f_1(\bx_t; \btheta_{t-1}^1) \right)  \right| \right] \\
& =     \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(r_t) \sim \cald} \left[ \left|f_2 \left( \bx_t ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_t - f_1(\bx_t; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \right]  \\
& \leq \underbrace{ \frac{1}{t}\sum_{\tau=1}^t \left|f_2 \left( \bx_t ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_t - f_1(\bx_t; \widehat{\btheta}_{\tau-1}^1) \right)  \right|}_{I_3}   + ( 1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}   ~.
\end{aligned}
\]
}


For $I_3$, according to Lemma \ref{lemma:caogeneli},  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$ , we have 
\begin{equation} \label{eq:f12upper}
\begin{aligned}
  & \frac{1}{t}\sum_{\tau=1}^t \left|  f_2 ( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|   \\
   & \leq   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|}_{I_4}  + \frac{3L}{\sqrt{2t}}~.
\end{aligned}
\end{equation}
 For $I_4$, according to  Lemma \ref{lemma:zhu} (1), these exists   $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0  \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, 
such that
\begin{equation} \label{eq:convegene}
\begin{aligned}
 &\frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \\
&\leq  \frac{1}{t} \sqrt{t} \sqrt{ \underbrace{ \sum_{\tau=1}^t \left(   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2}_{I_5} } \\
&\leq  \frac{1}{\sqrt{t}}\sqrt{ \underbrace{2\epsilon}_{I_5}}~, 
\end{aligned}
\end{equation}
where $I_5$ follows by a direct application of  Lemma \ref{lemma:zhu} (1) by defining the loss $\mathcal{L}(\widetilde{\btheta}^2) =\frac{1}{2}\sum_{\tau=1}^t \left(   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2 \leq \epsilon$. 

Combining Eq.(\ref{eq:main}), Eq.(\ref{eq:f12upper}) and Eq.(\ref{eq:convegene}), with probability $(1-3\delta)$ we have 
%\abcomment{need to mention expectation over $\btheta^1,\btheta^2$}
\begin{equation}\label{eq:fincon}
\begin{aligned}
 & \bbe_{(\bx, r) \sim \cald}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| | \{ \bx_{\tau}, r_{\tau}\}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~.
 \end{aligned}
\end{equation}
where the expectation over $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.

Then, applying union bound and rescaling the $\delta$ complete the proof. \qed







\begin{corollary}\label{corollary:main1} 
Given $\delta, \epsilon \in (0, 1), \rho \in (0, \mathcal{O}(\frac{1}{L}))$, suppose $m, \eta_1, \eta_2, K_1, K_2$ satisfy the conditions in Eq. (\ref{eq:condi}). Then, with probability at least $1- \delta$,  for any round $\tau \in [t], i \in [n]$, there exists a constant $c_1 > 0$, such that it holds uniformly for Algorithm \ref{alg:main} that
\begin{equation}\label{eq:lemmamain}
\begin{aligned}
\underset{\bx_{t,i}, i \in [n]}{\bbe} \bigg[ \max_{i \in [n]} \Bigg( \underset{r_{t,i}}{\bbe}   &  \bigg[ \Big | f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t,i}; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right) \Big |   \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i}  \bigg] \Bigg) \Bigg]\\
& \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}} ,
\end{aligned}
\end{equation}
where $ \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} $ are the data collected up to round $t-1$ and
the expectation is taken over $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.
\end{corollary}

\proof
This a direct corollary of Lemma \ref{lemma:main1}.
According to Eq. (\ref{eq:fincon}),
with probability $1-3\delta$,  given $ (\bx, r) \sim \cald$, we have 
%\abcomment{need to mention expectation over $\btheta^1,\btheta^2$}
\begin{equation}
\begin{aligned}
 & \underset{ \bx }{\bbe}  ~ \underset{r}{\bbe}     ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right|  \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~.
 \end{aligned}
\end{equation}


Then, in round $t$,  applying the union bound, for $(\bx_{t,i}, r_{t,i}) \sim \cald, \forall i \in [n]$,  with probability $1 - 3n \delta$, we have

\begin{equation}
\begin{aligned}
\forall i \in [n],  \ \  & \underset{\bx_{t,i}}{\bbe}  ~ \underset{r_{r,i}}{\bbe}     ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx_{t, i} ; \btheta_{t-1}^2\right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right)  \right|  \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~,
 \end{aligned}
\end{equation}

which is equal to
\begin{equation}
\begin{aligned}
\underset{\bx_{t,i}, i \in [n]}{\bbe} \bigg[ \max_{i \in [n]} \bigg( \underset{r_{t,i}}{\bbe}~ \underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}  &  \left[ \left|f_2 \left( \bx_{t,i} ; \btheta_{t-1}^2\right) - \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right)  \right|   \mid  \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}, \bx_{t,i}  \right]  \bigg) \bigg]\\
& \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}} + (1 +   2 \xi ) \sqrt{ \frac{2 \log (1 /\delta) }{t}}.
 \end{aligned}
\end{equation}
Then, apply union bound for any round $\tau \in [t]$, to help the proof for Theorem \ref{theo1}. Rescaling the $\delta$ and replacing $f_2$ with the formal form complete the proof.


\iffalse
Note that the same analysis can be done conditioned on $\bx := \bx_{t,i}$ such that 
\begin{equation*}
%\label{eq:fincon2}
\begin{aligned}
\bbp \left( \bbe_{r_{t,i} } ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| \mid \bx_{t,i} \right] \right. \geq  \left. \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta') }{t}} \right) \leq 3\delta'~.
 \end{aligned}
\end{equation*}
Since $\bx_{t,i}, i \in [n]$ are drawn i.i.d.,~ by union bound and using $\delta = t n \delta'$, with probability $(1-\delta)$ we have
\begin{equation*}
%\label{eq:fincon2}
\begin{aligned}
\max_{i \in [n]} \left( \bbe_{r_{t,i} } ~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx ; \btheta_{t-1}^2\right) - \left(r - f_1(\bx; \btheta_{t-1}^1) \right)  \right| \mid \bx_{t,i} \right] \right) \leq  \sqrt{\frac{ 2\epsilon}{t}} + \frac{3L}{\sqrt{2t}}  + (1 + 2 \xi) \sqrt{ \frac{2 \log (t n/\delta) }{t}} ~.
 \end{aligned}
\end{equation*}
Taking expectation w.r.t.~$\bx_{t,i}, i\in [n]$ completes the proof. 
\fi
\qed


%\abcomment{Have not explained why we need to take union bound over $t$, will be good to add that. Note that we have not maintianed the conditioning w.r.t.~the history $F_{\tau}$ through the proof, will also be good to do that.}












\begin{lemma} \label{lemma:a}
 
 Let $f(\cdot; \widehat{\btheta}_t)$ follow the stochastic gradient descent of $f_1$ or $f_2$ in Algorithm \ref{alg:main}.
 Suppose $m, \eta_1, \eta_2$ satisfy the conditions in Eq. (\ref{eq:condi}).  With probability at least $1 - \delta$, for any $\bx$ with $\|\bx\|_2 = 1$ and $t \in [T]$, it holds that
\[
| f(\bx; \widehat{\btheta}_t)| \leq  \mathcal{O}(1) +  \mathcal{O} \left( \frac{t^3n L \log m}{ \rho \sqrt{m} } \right) + \mathcal{O} \left(  \frac{t^4 n L^2  \log^{11/6} m}{ \rho  m^{1/6}}\right).
\]
\end{lemma}



%\begin{prove*}
\proof Considering an inequality $ |a - b| \leq c$, we have $|a| \leq |b| + c$. 
Let $\btheta_0$ be randomly initialized. Then applying  Lemma \ref{lemma:gu} (1),  for any $\bx \sim \mathcal{D}, \|\bx \|_2 = 1$ and $ \|\widehat{\btheta}_t - \btheta_0\| \leq w$,  we have 
\begin{equation}
\begin{aligned}
|f(\bx; \widehat{\btheta}_t) | &\leq  | f(\bx; \btheta_0)| +  |\langle  \triangledown_{\btheta_0}f(\bx_i; \btheta_0), \widehat{\btheta}_t - \btheta_0   \rangle  | +   \mathcal{O} ( L^2 \sqrt{m \log(m)}) \|\widehat{\btheta}_t - \btheta_0 \|_2 w^{1/3} \\
&  \leq \underbrace{\mathcal{O}(1)}_{I_0}  +  \underbrace{  \|  \triangledown_{\btheta_0}f(\bx_i; \btheta_0)  \|_2 \| \widehat{\btheta}_t - \btheta_0  \|_2}_{I_1}  + \mathcal{O} ( L^2 \sqrt{m \log(m)}) \|\widehat{\btheta}_t - \btheta_0 \|_2 w^{1/3} \\
& \leq \mathcal{O}(1) +  \underbrace{  \mathcal{O} (L) \cdot  \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)}_{I_2} + \underbrace{   \mathcal{O} \left( L^2 \sqrt{m \log(m)} \right) \cdot  \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)^{4/3} }_{I_3}  \\
&  =  \mathcal{O}(1) +  \mathcal{O} \left( \frac{t^3 L \log m}{ \rho \sqrt{m} } \right) + \mathcal{O} \left(  \frac{t^4 L^2  \log^{11/6} m}{ \rho  m^{1/6}}\right)
\end{aligned}
\end{equation}
where: $I_0$ is based on the Lemma \ref{lemma:zhu} (3);
$I_1$ is an application of Cauchy–Schwarz inequality; $I_2$ is according to  Lemma \ref{lemma:zhu} (2) and (3) in which $\widehat{\btheta}_t$ can be considered as one step gradient descent; $I_3$ is due to Lemma \ref{lemma:zhu} (2).

Then, the proof is completed. \qed
%\end{prove*}












\begin{lemma} \label{lemma:zhu}
Given a constant $0 < \epsilon < 1$, suppose $m \geq  \widetilde{\Omega}   \left ( \text{poly}(T, n, L, \rho^{-1}) \cdot    e^{\sqrt{\log 1/\delta }}  \right ) $, the learning rate $\eta = \Omega(\frac{\rho}{ \text{poly} (t ,n, L) m} ) $, the number of iterations $K = \Omega (\frac{\text{poly}(t, n, L)}{\rho^2} \cdot \log \epsilon^{-1})$. Then, with probability at least $1 - \delta$,  starting from random initialization $\btheta_0$, 
\begin{enumerate}[label=(\arabic*)]
    \item (Theorem 1 in \citep{allen2019convergence}) 
    In round $t \in [T]$, given the collected data $\{\bx_\tau, r_\tau\}_{i=\tau}^{t}$, the loss function is defined as:
    $\mathcal{L}(\btheta) = \frac{1}{2} \sum_{\tau = 1}^{t}   \left( f(\bx_{\tau}; \btheta) - r_\tau \right)^2$.
    Then,  there exists  $\widetilde{\btheta}$  satisfying $\|\widetilde{\btheta} - \btheta_0\|_2 \leq \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)$, such that
    $ \mathcal{L}(\widetilde{\btheta}) \leq \epsilon $ in $K = \Omega (\frac{\text{poly}(t, n, L)}{\rho^2} \cdot \log \epsilon^{-1})$ iterations;\\
    \item (Theorem 1 in \citep{allen2019convergence}) For any $k \in [K]$, it holds uniformly that
    $
    \|\btheta^{(k)}_t - \btheta_0\|_2 \leq \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)
    $;
    \item Following the initialization, it holds that
    \[
     \|   \triangledown_{\btheta_0 }f(\bx_i; \btheta_0)  \|_2 \leq \mathcal{O} (L),   \    \   \
      |  f(\bx_i; \btheta_0)  | \leq \mathcal{O} (1)
    \]
\end{enumerate}
where $\btheta^{(k)}_t$ represents the parameters of $f$ after $k \in [K] $ iterations if gradient descent in round $t$.
\end{lemma}

%\begin{prove*}
\proof 
Note that the output dimension $d$ in \citep{allen2019convergence} is removed because the output of network function in this paper always is a scalar.
For (1) and (2),  the only different setting from \citep{allen2019convergence} is that the initialization of last layer $\bw_{L} \sim \mathcal{N}(0, \frac{2}{m})$ in this paper while $\bw_{L} \sim \mathcal{N}(0, \frac{1}{d})$ in \citep{allen2019convergence}. Because $d =1$ and $m > d$ here, the upper bound in \citep{allen2019convergence} still holds for $\bw_L$: with probability at least $1 - \exp{(- \Omega(m/L))}, \|\bw_L\|_F \leq \sqrt{m/d}$. Therefore, it is easy to verify that (1) and (2) still hold for the initialization of this paper.

For (3), based on Lemma 7.1 in \cite{allen2019convergence}, we have $ |  f(\bx_i; \btheta_0)  | \leq \mathcal{O} (1)$. Denote by $D$ the ReLU function.  For any $l \in [L]$, 
\[
\|\triangledown_{W_l}f(\bx_i; \btheta_0)\|_F \leq   \|\bw_L D \bw_{L-1} \cdots D \bw_{l+1}\|_F \cdot \| D \bw_{l+1} \cdots \bx \|_F \leq  \mathcal{O}(\sqrt{L}) 
\] 
where the inequality is according to Lemma 7.2 in \cite{allen2019convergence}. Therefore, we have $ \|   \triangledown_{\btheta_0 }f(\bx_i; \btheta_0)  \|_2 \leq \mathcal{O} (L) $. \qed 
%\end{prove*}




\begin{lemma} [Lemma 4.1, \citep{cao2019generalization}]  \label{lemma:gu} 
Suppose $ \mathcal{O}( m^{-3/2} L^{-3/2} [ \log (TnL^2/\delta) ]^{3/2}  )   \leq w \leq  \mathcal{O} (L^{-6}[\log m]^{-3/2} )$. Then,
with probability at least $1- \delta$ over randomness of $\btheta_0$, for any $ t \in [T], \|\bx \|_2 =1 $, and $\btheta, \btheta'$
satisfying $\| \btheta - \btheta_0 \|_2 \leq w$ and $\| \btheta' - \btheta_0 \|_2 \leq w$
, it holds uniformly that
\begin{enumerate}[label=(\arabic*)]
 \item $
| f(\bx_i; \btheta) - f(\bx_i; \btheta') -  \langle  \triangledown_{\btheta'}f(\bx_i; \btheta'), \btheta - \btheta'    \rangle    | \leq \mathcal{O} (w^{1/3}L^2 \sqrt{m \log(m)}) \|\btheta - \btheta'\|_2
$
\item $  \| \triangledown_{\btheta}f(\bx; \btheta)\|_2  \leq \mathcal{O}(\sqrt{mL})$.
\end{enumerate}
\end{lemma}


\begin{lemma} \label{lemma:caogeneli}
For any $\delta > 0$, suppose
\[
m > \tilde{\mathcal{O}}\left(  \text{poly} (T, n, \rho^{-1}, L, \log (1/\delta) \cdot e^{\sqrt{ \log 1/\delta}}) \right), \ \ \nu = \tilde{\Theta}(t^6/\delta^2).  
\]
Then, with probability at least $1 - \delta$, setting $\eta_2 = \Theta( \frac{ \nu}{\sqrt{2} t m})$ for algorithm \ref{alg:main},   for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$  such that
\[
\begin{aligned}
\sum_{\tau=1}^t \left|   f_2 \left( \frac{\triangledown_{\widehat{\btheta}_{\tau-1}^1 }f_1(\bx_\tau ; \widehat{\btheta}_{\tau-1}^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_{\tau-1}^2  \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| \\
\leq   \sum_{\tau=1}^t \left|   f_2  \left( \frac{\triangledown_{\widehat{\btheta}_{\tau-1}^1}f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_{t}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| + \frac{3L\sqrt{t} }{\sqrt{2}}\\
\end{aligned}
\]
\end{lemma}
\begin{proof}
This is a direct application of Lemma 4.3 in \citep{cao2019generalization} by setting $R = \frac{t^3}{\rho} \log m,  \epsilon = \frac{LR}{ \sqrt{2\nu t}}$,  and $ \nu = R^2$.
We set $L_\tau( \widehat{\btheta}_{\tau -1}^2 ) =  \left |  f_2 ( \triangledown_{\widehat{\btheta}_{\tau-1}^1} f_1  ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| $.
Based on Lemma \ref{lemma:zhu} (2), for any $\tau \in [t]$, we have 
\[ 
\|\widehat{\btheta}_{\tau}^2 - \widehat{\btheta}_{\tau-1}^2\|_2 \leq  \| \widehat{\btheta}_{\tau}^2 - \btheta_0 \|_2 + \| \btheta_0 -   \widehat{\btheta}_{\tau-1}^2 \|_2 \leq \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m).
\]
Then, according to Lemma 4.3 in \citep{cao2019generalization}, then,  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, we have 
\begin{equation}
\sum_{\tau=1}^t  L_\tau( \widehat{\btheta}_{\tau -1}^2 ) \leq \sum_{\tau=1}^t L_\tau( \widetilde{\btheta}^2) + 3 t \epsilon.
\end{equation}
Then, replacing $\epsilon$ completes the proof.
\end{proof}







==> analysis1_new2.tex <==
%\newpage

\section{Proof of Theorem \ref{theo1}} \label{sec:the1p}

In this section, we provide the proof of Theorem \ref{theo1} and related lemmas.


\proof
For brevity, for the selected arm $\bx_t$ in round $t$, let $h(\bx_t)$ be its expected reward and $ \bx_t^\ast = \arg \max_{i \in [n]} h(\bx_{t,i})$ be the optimal arm in round $t$.

Note that $(\bx_{t,i}, r_{t,i}) \sim \cald$, for each $i \in [n]$. Then, the expected regret of round $t$ is given by
\begin{equation}
\begin{aligned}
\mathbf{R}_t 
& =  \underset{(\bx_{t,i}, r_{t,i}),  i \in [n] }{\bbe} [ r^\ast_t - r_t | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}]\\
%& =  \underset{(\bx_{t,i}, r_{t,i}),  i \in [n] }{\bbe} [ r^\ast_t - r_t | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}]\\
& = \bbe_{\bx_{t,i}, i \in [n]} [ h(\bx_t^\ast) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}  ]   \\
&  =  \bbe_{\bx_{t,i}, i \in [n]}[h(\bx_t^\ast)  - f_3(\bx_t)  + f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] \\
&  \leq \bbe_{\bx_{t,i}, i \in [n]}[\underbrace{  h(\bx_t^\ast) - f_3(\bx_t^\ast) +  f_3(\bx_t)  - f_3(\bx_t)  }_{I_1} +   f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}]  \\
& =  \bbe_{\bx_{t,i}, i \in [n]}[h(\bx_t^\ast) - f_3(\bx_t^\ast) + f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] \\
& =  \bbe_{\bx_{t,i}, i \in [n]}[h(\bx_t^\ast) - f_3(\bx_t^\ast) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] + \bbe_{\bx_{t,i}, i \in [n]}[f_3(\bx_t) - h(\bx_t) | \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1}] \\
& =  \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe} 
  \left[  \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t}^\ast; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t}^\ast - f_1(\bx_{t}^\ast; \btheta_{t-1}^1) \right) \right | \mid \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
& \ \ \ +  \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe} 
  \left[  \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t}; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t} - f_1(\bx_{t}; \btheta_{t-1}^1) \right) \right | \mid \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\ 
\end{aligned}
\end{equation}
where $I_1$ is because $f_3(\bx_t) = \max_{i \in [n]}f_3(\bx_{t,i})$ and $f_3(\bx_t) - f_3(\bx_t^\ast) \geq 0$, and (a) follows by Jensen's inequality. 

%\ban{Maybe, it is better to remove $\mathbf{X}_t$ in the condition ?}




%\ban{I have a question, if $\bbe[ \left(r_{t,i} - f_1(\bx_{t,i}; \btheta_{t-1}^1) \right) | \bx_{t,i}] =  \bbe_{\bx \sim \cald} [ \left(r - f_1(\bx; \btheta_{t-1}^1) \right) ] $ ?}



%\abcomment{If we want to be more rigorous, the above analysis should also be conditioned on the history $(\x_{\tau},r_{\tau}), \tau =1,\ldots,t-1$ because that conditioning shows up below.}

Because, for each $i \in [n]$, $(\bx_{t,i}, r_{t,i}) \sim \cald$, applying Lemma \ref{lemma:main1} and Corollary \ref{corollary:main1},
%to $(\bx_{t,i}, r_{t,i}), \forall i \in [n]$,  
with probability at least $(1-\delta)$, we have
\begin{equation}
\mathbf{R}_t  \leq  2 \left(
\sqrt{\frac{ 2\epsilon}{t}} + \calo \left( \frac{3L}{\sqrt{2t}}\right) + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}}  \right)~,
\end{equation}
where we apply the union bound over round $\tau, \forall \tau \in [t]$ to make Lemma \ref{lemma:main1} and Corollary \ref{corollary:main1} hold for each round $\tau, \tau \in [t]$.

Then expected regret of $T$ rounds is computed by
\begin{equation}
\begin{aligned}
\mathbf{R}_T & = \sum_{t =1}^T \mathbf{R}_t\\
 & \leq 2 \sum_{t =1}^T   \left(
\sqrt{\frac{ 2\epsilon}{t}} + \calo \left( \frac{3L}{\sqrt{2t}} \right) + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn) /\delta) }{t}}  \right)  \\
& \leq \underbrace{  (2\sqrt{T} -1) 2\sqrt{2 \epsilon} + 
(2\sqrt{T} -1) 3\sqrt{2} \calo(L) +  
2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} }_{I_2} \\
&= (2 \sqrt{T} -1 ) ( 2\sqrt{2 \epsilon} + 3\sqrt{2}\calo(L)) +  2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}
\end{aligned}
\end{equation}
where  $I_2$ is because $\sum_{t=1}^T \frac{1}{\sqrt{t}}  \leq  \int_{1}^T   \frac{1}{\sqrt{t}}  \ dx  +1 =  2 \sqrt{T} -1$ \citep{chlebus2009approximate}.

According to Lemma \ref{lemma:zhu} (1),  with probability at least $1 - \delta$, when $\epsilon \leq  1/T$, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +  (2\sqrt{T} -1) 3\sqrt{2} \calo(L) +    2 (1 + 2\xi) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}, 
\end{equation}
As the choice of $m$, we have $\xi \leq \mathcal{O}(1)$. Therefore, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +  (2\sqrt{T} -1) 3\sqrt{2} \calo(L)  +  \mathcal{O} \left((2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} \right).
\end{equation}
The proof is completed. \qed
%\end{prove*}




\begin{lemma}\label{lemma:main1} [\textbf{Lemma \ref{lemma:main} restated}]
Given $\delta, \epsilon \in (0, 1), \rho \in (0, \mathcal{O}(\frac{1}{L}))$, suppose $m, \eta_1, \eta_2, K_1, K_2$ satisfy the conditions in Eq. (\ref{eq:condi}) and $(\bx_{\tau, i}, r_{\tau, i}) \sim \cald, \forall \tau \in [t], i \in [n]$. Let
\[
\bx_t = \arg \max_{\bx_{t, i}, i \in [n]} \left[ f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t,i}; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) + f_1(\bx_{t,i}; \btheta_{t-1}^1)  \right],
\]
and $r_t$ is the corresponding reward, given $(\bx_{t, i}, r_{t, i}), i \in [n]$.
Then, with probability at least $(1- \delta)$  over the random of the initialization, it holds that
 \begin{equation}\label{eq:lemmamain}
 \begin{aligned}
 \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe} 
 & \left[  \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t}; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t} - f_1(\bx_{t}; \btheta_{t-1}^1) \right) \right | \mid \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
 & \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} +  \calo \left( \frac{3L}{\sqrt{2t}} \right) + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn /\delta) ) }{t}} ,
 \end{aligned}
 \end{equation}
where  the expectation is also taken over  $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that are  uniformly drawn from $(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2), \tau \in [t-1]$.
\end{lemma}





%\abcomment{based on what we choose, the proof below will have to be mildly updated}

\proof 
In this proof, we consider the collected data of up to round $t-1$,  $\{\bx_\tau,  r_\tau \}_{\tau=1}^{t-1}$, as the training dataset and then obtain a generalization bound for it, inspired by \cite{cao2019generalization}.

%First, we focus on upper bounding the conditional expectation $\bbe_{r_{t,i}}[ \cdots | \bx_{t,i}]$ in \eqref{eq:lemmamain} with high probability.  

For convenience, we use $\bx := \bx_{t,i}, r := r_{t,i}$, noting that the same analysis holds for each $i \in [n]$. Using the Lemma \ref{lemma:gu} (2) and Lemma \ref{lemma:zhu} (2), for any $\tau \in [t-1]$, with probability at least $(1 -\delta)$ over the random initialization, given any $\bx \sim \cald_{\bx}$ and $\| \bx \|_2 \leq 1$,  we have  
%\abcomment{$t$ should be replaced by $\tau = 1,\ldots, t-1$ below, and the subsequent equations ... till we take the expectation over these}
%\abcomment{perhaps state the result for $\widehat{\btheta}^1_t$ since that is what we need later}
\[ \|\triangledown_{\widehat{\btheta}^1_\tau}f(\bx; \widehat{\btheta}^1_\tau)\|_2 \leq \mathcal{O}(\sqrt{mL}). 
\]
Now, consider the exploration network $f_2$.   Given any $\bx \sim \cald$ and $\| \bx \|_2 \leq 1$,  there must exist a constant $c_1$,  such that 
%\abcomment{again, for $\widehat{\btheta}^1_\tau$}
\begin{equation}
\left \| \frac{\triangledown_{\widehat{\btheta}_\tau^1}f_1(\bx; \widehat{\btheta}^1_\tau)}{c_1 \sqrt{mL}}  \right \|_2 \leq  1.
\end{equation}
  Then, applying Lemma \ref{lemma:a},  with probability at least $1-\delta$, for any $t \in [T]$,  we have 

\begin{equation} \label{eq:f2value}
 \left| f_2\left( \frac{\triangledown_{\widehat{\btheta}_\tau^1}f_1( \bx;  \widehat{\btheta}_\tau^1) }{c_1\sqrt{mL} }   ;\widehat{\btheta}_\tau^2\right) \right| \leq  \xi.
\end{equation}

Similarly, applying  Lemma \ref{lemma:a} again,  with probability at least $1-\delta$, for any $t \in [T]$,  we have 
%\abcomment{for $\widehat{\btheta}^1_\tau$} \abcomment{where is $\xi_1$ defined?}
\begin{equation} \label{eq:f1value}
|   f_1(\bx; \widehat{\btheta}_\tau^1 )  | \leq \xi
\end{equation}


Because for any $r \sim \cald$, $|r| \leq 1$, with Eq. (\ref{eq:f2value}) and (\ref{eq:f1value}), 
applying union bound, with probability at least $(1 - 2\delta)$ over the random initialization, we have 
\begin{equation} \label{eq:upperboundoff2}
 \left | f_2 \left( \frac{\triangledown_{ \widehat{ \btheta}_\tau^1 }f_1(\bx; \widehat{ \btheta}_\tau^1)}{c_1\sqrt{mL} }   ; \widehat{\btheta}_\tau^2\right)  -  (r -  f_1(\bx; \widehat{\btheta}_\tau^1 )) \right |  \leq 1  +  2\xi.
\end{equation}
Noting that \eqref{eq:upperboundoff2} is for $\bx = \bx_{\tau,i}$ for a specific $\tau \in [t], i \in [n]$. By union bound, \eqref{eq:upperboundoff2} holds $\forall \tau \in [t], i \in [n]$ with probability at least $(1-nt \delta)$. 
For brevity, let $f_2( \bx ;  \widehat{\btheta}_\tau^2)$ represent $f_2\left( \frac{\triangledown_{\widehat{\btheta}^1_\tau }f_1(\bx ; \widehat{\btheta}_\tau^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_\tau^2\right)$. 


Recall that, for each $\tau \in [t-1]$, 
%\abcomment{we may have used both $\tau \in [t-1]$ and $\tau \in [t]$, pls check}
$\widehat{\btheta}_\tau^1$ and $\widehat{\btheta}_\tau^2$ are the parameters training on $\{\bx_{\tau'}, r_{\tau'} \}_{\tau'=1}^\tau$ according to Algorithm \ref{alg:main}.
In round $\tau \in [t]$, let $ \bx_\tau = \arg \max_{\bx_{\tau, i}, i \in [n]} [ f_1(\bx_{\tau, i}; \btheta_{\tau-1}^1)  + f_2(\bx_{\tau, i}; \btheta_{\tau-1}^2 ) ], $ given $(\bx_{\tau, i}, r_{\tau, i} ) \sim \cald, i \in [n]$.  
Then, we 
define 
\begin{equation} 
\begin{aligned}
V_{\tau} =& \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{\bbe}
\left[ \left|f_2( \bx_{\tau} ; \widehat{\btheta}_{\tau-1}^2) - \left(r_\tau - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right] \\ 
 &- \left|f_2( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right) \right|~.
\end{aligned}
\end{equation}
%\abcomment{$V_{\tau}$ should be based on $(\bx_{\tau, i_{\tau}}, r_{\tau, i_{\tau}})$ where $i_{\tau}$ is a function of $\bx_{\tau,i}, i \in [n]$, and the analysis should be conditioned on this. Lets check if this works, and if the analysis can be done conditioned on $\bx_{\tau,i}, i \in [n]$.}

Then, as $(\bx_{\tau,i},r_{\tau,i}) \sim \cald, i \in [n]$, based on the definition of $(\bx_{\tau}, r_{\tau}),$ we have
 \begin{equation} \label{eq:vexp0}
 \begin{aligned}
 \bbe[  V_{\tau} | \mathbf{F}_{\tau-1}] & =  \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{\bbe}
 \left[ \left|f_2\left(  \bx_{\tau} ; \widehat{ \btheta}_{\tau-1}^2\right) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \mid \mathbf{F}_{\tau-1} \right]  \\
& \quad -   \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{  \bbe}
\left[  \left|f_2 \left( \bx_{\tau} ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right) \right| |  \mathbf{F}_{\tau-1} \right] \\
& = 0~,
\end{aligned}
 \end{equation}
where $ \mathbf{F}_{\tau-1}$ denotes the $\sigma$-algebra generated by the history ${\cal H}_{\tau-1} = \{ \bx_{\tau'}, r_{\tau'}\}_{\tau' = 1}^{\tau-1}$. 
%Note that $(\bx_{\tau}, r_{\tau}) \sim D$.

Moreover, we have
\[
\begin{aligned}
\frac{1}{t} \sum_{\tau=1}^t  V_{\tau} 
& =  \frac{1}{t}  \sum_{\tau=1}^t  
\underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{\bbe}
\left[ \left|f_2( \bx_{\tau} ; \widehat{\btheta}_{\tau-1}^2) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right]  \\
& \quad - \frac{1}{t}  \sum_{\tau=1}^t \left|f_2\left(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^2\right) - \left(r_{\tau} - f_1(\bx_{\tau};  \widehat{\btheta}_{\tau-1}^1) \right) \right| 
\end{aligned}
\] 


Since $\{V_{\tau}\}_{\tau = 1}^t$ is a martingale difference sequence, following Lemma 1 in \citep{cesa2004generalization}, applying the Hoeffding-Azuma inequality, 
%to the bounded random variables $V_{1}, \dots, V_{t} $,  
with probability at least $1 - 2\delta$,  we have 
\begin{equation}
\begin{aligned}
    \bbp \left[  \frac{1}{t}  \sum_{\tau=1}^t  V_{\tau}  -   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t  \bbe[ V_{\tau} | \mathbf{F}_{\tau} ] }_{I_1}   >  \underbrace{ ( 1 +  2 \xi)}_{I_2} \sqrt{ \frac{2 \log (1/\delta)}{t}}  \right] &\leq \delta  \\
 \Rightarrow  \qquad  \qquad   \bbp\left[  \frac{1}{t}  \sum_{\tau=1}^t  V_{\tau}   >  ( 1 +  2\xi) \sqrt{ \frac{2 \log (1/\delta)}{t}}  \right] & \leq \delta  ~,
\end{aligned}  
\label{eq:pppuper}
\end{equation}
where $I_1 = 0 $ according to Eq.(\ref{eq:vexp0}) and $I_2$ is because of Eq.(\ref{eq:upperboundoff2}).

According to Algorithm \ref{alg:main}, $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.
Thus, with probability $1 -3\delta$, we have 
\begin{equation}\label{eq:main}
\begin{aligned}
& \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx_t ; \btheta_{t-1}^2\right) - \left(r_t - f_1(\bx_t; \btheta_{t-1}^1) \right)  \right| \right] \\
& =     \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]} \left[ \left|f_2 \left( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \right]  \\
& \leq \underbrace{ \frac{1}{t}\sum_{\tau=1}^t \left|f_2 \left( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right)  \right|}_{I_3}   + ( 1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}   ~.
\end{aligned}
\end{equation}

For $I_3$, according to Lemma \ref{lemma:caogeneli},  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$ , we have 
\begin{equation} \label{eq:f12upper}
\begin{aligned}
  & \frac{1}{t}\sum_{\tau=1}^t \left|  f_2 ( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|   \\
   & \leq   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|}_{I_4}  + \calo\left( \frac{3L}{\sqrt{2t}} \right) ~.
\end{aligned}
\end{equation}
 For $I_4$, according to  Lemma \ref{lemma:zhu} (1), these exists   $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0  \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, 
such that
\begin{equation} \label{eq:convegene}
\begin{aligned}
 &\frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \\
&\leq  \frac{1}{t} \sqrt{t} \sqrt{ \underbrace{ \sum_{\tau=1}^t \left(   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2}_{I_5} } \\
&\leq  \frac{1}{\sqrt{t}}\sqrt{ \underbrace{2\epsilon}_{I_5}}~, 
\end{aligned}
\end{equation}
where $I_5$ follows by a direct application of  Lemma \ref{lemma:zhu} (1) by defining the loss $\mathcal{L}(\widetilde{\btheta}^2) =\frac{1}{2}\sum_{\tau=1}^t \left(   f_2 ( \bx_\tau ; \widetilde{\btheta}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2 \leq \epsilon$. 

Combining Eq.(\ref{eq:main}), Eq.(\ref{eq:f12upper}) and Eq.(\ref{eq:convegene}), with probability $(1-3\delta)$ we have 
%\abcomment{need to mention expectation over $\btheta^1,\btheta^2$}
\begin{equation}\label{eq:fincon}
\begin{aligned}
 & \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}   \left[\left|f_2 \left( \bx_t ; \btheta_{t-1}^2\right) - \left(r_t - f_1(\bx_t; \btheta_{t-1}^1) \right)  \right| | \{ \bx_{\tau}, r_{\tau}\}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} + \calo \left( \frac{3L}{\sqrt{2t}} \right)  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~.
 \end{aligned}
\end{equation}
where the expectation over $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that is uniformly drawn from $\{(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2)\}_{\tau = 0}^{t-1}$.

Then, applying union bound to $t, n$ and rescaling the $\delta$ complete the proof. \qed







\begin{corollary}\label{corollary:main1} 
Given $\delta, \epsilon \in (0, 1), \rho \in (0, \mathcal{O}(\frac{1}{L}))$, suppose $m, \eta_1, \eta_2, K_1, K_2$ satisfy the conditions in Eq. (\ref{eq:condi}) and $(\bx_{\tau, i}, r_{\tau, i}) \sim \cald, \forall \tau \in [t], i \in [n]$. Let
\[
\bx_t^\ast = \arg \max_{\bx_{t, i}, i \in [n]} \left[ h(\bx_{t,i})  \right],
\]
and $r_t^\ast$ is the corresponding reward, given $(\bx_{t, i}, r_{t, i}), i \in [n]$.
Then, with probability at least $(1- \delta)$  over the random of the initialization, it holds that
 \begin{equation}\label{eq:lemmamain}
 \begin{aligned}
 \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe} 
 & \left[  \left| f_2 \left( \frac{\triangledown_{\btheta^1_{t-1} }f_1(\bx_{t}^\ast; \btheta^1_{t-1})}{c_1 \sqrt{mL}} ; \btheta_{t-1}^2 \right) - \left(r_{t}^\ast - f_1(\bx_{t}^\ast; \btheta_{t-1}^1) \right) \right | \mid \{\bx_\tau,  r_\tau \}_{\tau = 1}^{t-1} \right] \\
 & \qquad \qquad \leq \sqrt{\frac{ 2\epsilon}{t}} + \calo \left( \frac{3L}{\sqrt{2t}} \right) + (1 +   2 \xi ) \sqrt{ \frac{2 \log ( \mathcal{O}(tn /\delta) ) }{t}} ,
 \end{aligned}
 \end{equation}
where  the expectation is also taken over  $(\btheta_{t-1}^1, \btheta_{t-1}^2 )$ that are  uniformly drawn from $(\widehat{\btheta}_{\tau}^1, \widehat{\btheta}_{\tau}^2), \tau \in [t-1]$.
\end{corollary}

\proof
This a direct corollary of Lemma \ref{lemma:main1}.





In round $t$, let $ \bx_t^\ast = \arg \max_{\bx_{t, i}  i \in [n]} [h(\bx_{t,i}) ], $ given $(\bx_{t, i}, r_{t, i} ) \sim \cald, i \in [n]$.  
Then, we 
define 
\begin{equation} 
\begin{aligned}
V_{t} =& \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}
\left[ \left|f_2( \bx_t^\ast ; \widehat{\btheta}_{t-1}^2) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{t-1}^1) \right)  \right| \right] \\ 
 &- \left|f_2( \bx_t^\ast ; \widehat{\btheta}_{t-1}^2) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{t-1}^1) \right) \right|~.
\end{aligned}
\end{equation}


Then, as $(\bx_{t,i},r_{t,i}) \sim \cald, i \in [n]$, we have
 \begin{equation} \label{eq:vexp0}
 \begin{aligned}
 \bbe[  V_{t} | \mathbf{F}_{t-1}] & =  \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}
 \left[ \left|f_2\left(  \bx_t^\ast ; \widehat{ \btheta}_{t-1}^2\right) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{t-1}^1) \right)  \right| \mid \mathbf{F}_{t-1} \right]  \\
& \quad -   \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{  \bbe}
\left[  \left|f_2 \left( \bx_t^\ast ; \widehat{\btheta}_{t-1}^2 \right) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{t-1}^1) \right) \right| \mid  \mathbf{F}_{t-1} \right] \\
& = 0~,
\end{aligned}
 \end{equation}
where $ \mathbf{F}_{t-1}$ denotes the $\sigma$-algebra generated by the history ${\cal H}_{t-1} = \{ \bx_{\tau'}, r_{\tau'}\}_{\tau' = 1}^{t-1}$. 


In round $\tau \in [t-1]$, let $ \bx_\tau = \arg \max_{\bx_{\tau, i}, i \in [n]} [ f_1(\bx_{\tau, i}; \btheta_{\tau-1}^1)  + f_2(\bx_{\tau, i}; \btheta_{\tau-1}^2 ) ], $ given $(\bx_{\tau, i}, r_{\tau, i} ) \sim \cald, i \in [n]$.  
Then, we 
define 
\begin{equation} 
\begin{aligned}
V_{\tau} =& \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{\bbe}
\left[ \left|f_2( \bx_{\tau} ; \widehat{\btheta}_{\tau-1}^2) - \left(r_\tau - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right] \\ 
 &- \left|f_2( \bx_\tau ; \widehat{\btheta}_{\tau-1}^2) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right) \right|~.
\end{aligned}
\end{equation}
%\abcomment{$V_{\tau}$ should be based on $(\bx_{\tau, i_{\tau}}, r_{\tau, i_{\tau}})$ where $i_{\tau}$ is a function of $\bx_{\tau,i}, i \in [n]$, and the analysis should be conditioned on this. Lets check if this works, and if the analysis can be done conditioned on $\bx_{\tau,i}, i \in [n]$.}

Then, as $(\bx_{\tau,i},r_{\tau,i}) \sim \cald, i \in [n]$, based on the definition of $(\bx_{\tau}, r_{\tau}),$ we have
 \begin{equation} \label{eq:vexp0}
 \begin{aligned}
 \bbe[  V_{\tau} | \mathbf{F}_{\tau-1}] & =  \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{\bbe}
 \left[ \left|f_2\left(  \bx_{\tau} ; \widehat{ \btheta}_{\tau-1}^2\right) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \mid \mathbf{F}_{\tau-1} \right]  \\
& \quad -   \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{  \bbe}
\left[  \left|f_2 \left( \bx_{\tau} ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_{\tau} - f_1(\bx_{\tau}; \widehat{\btheta}_{\tau-1}^1) \right) \right| |  \mathbf{F}_{\tau-1} \right] \\
& = 0~,
\end{aligned}
 \end{equation}
where $ \mathbf{F}_{\tau-1}$ denotes the $\sigma$-algebra generated by the history ${\cal H}_{\tau-1} = \{ \bx_{\tau'}, r_{\tau'}\}_{\tau' = 1}^{\tau-1}$. 
%Note that $(\bx_{\tau}, r_{\tau}) \sim D$.











\iffalse
In round $\tau \in [t]$, let $ \bx_\tau^\ast = \arg \max_{\bx_{\tau, i}  i \in [n]} [h(\bx_{\tau,i}) ], $ given $(\bx_{\tau, i}, r_{\tau, i} ) \sim \cald, i \in [n]$.  
Then, we 
define 
\begin{equation} 
\begin{aligned}
V_{\tau} =& \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}
\left[ \left|f_2( \bx_t^\ast ; \widehat{\btheta}_{\tau-1}^2) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \right] \\ 
 &- \left|f_2( \bx_t^\ast ; \widehat{\btheta}_{\tau-1}^2) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right|~.
\end{aligned}
\end{equation}
%\abcomment{$V_{\tau}$ should be based on $(\bx_{\tau, i_{\tau}}, r_{\tau, i_{\tau}})$ where $i_{\tau}$ is a function of $\bx_{\tau,i}, i \in [n]$, and the analysis should be conditioned on this. Lets check if this works, and if the analysis can be done conditioned on $\bx_{\tau,i}, i \in [n]$.}

Then, as $(\bx_{\tau,i},r_{\tau,i}) \sim \cald, i \in [n]$, we have
 \begin{equation} \label{eq:vexp0}
 \begin{aligned}
 \bbe[  V_{\tau} | \mathbf{F}_{\tau-1}] & =  \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{\bbe}
 \left[ \left|f_2\left(  \bx_t^\ast ; \widehat{ \btheta}_{\tau-1}^2\right) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{\tau-1}^1) \right)  \right| \mid \mathbf{F}_{\tau-1} \right]  \\
& \quad -   \underset{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]}{  \bbe}
\left[  \left|f_2 \left( \bx_t^\ast ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_t^\ast - f_1(\bx_t^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right| \mid  \mathbf{F}_{\tau-1} \right] \\
& = 0~,
\end{aligned}
 \end{equation}
where $ \mathbf{F}_{\tau-1}$ denotes the $\sigma$-algebra generated by the history ${\cal H}_{\tau-1} = \{ \bx_{\tau'}, r_{\tau'}\}_{\tau' = 1}^{\tau-1}$. 
%Note that $(\bx_{\tau}, r_{\tau}) \sim D$.

\fi

Therefore,  $\{V_{\tau}\}_{\tau = 1}^t$ is a martingale difference sequence.


Similarly, applying the Hoeffding-Azuma inequality to $V_{\tau}$, 
%to the bounded random variables $V_{1}, \dots, V_{t} $,  
with probability at least $1 - 2\delta$,  we have 

\begin{equation}
\begin{aligned}
& \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}~\underset{(\btheta_{t-1}^1, \btheta_{t-1}^2 )}{\bbe}   \left[\left|f_2 \left( \bx_t^\ast ; \btheta_{t-1}^2\right) - \left(r_t^\ast - f_1(\bx_t^\ast; \btheta_{t-1}^1) \right)  \right| \right] \\
& =     \frac{1}{t} \sum_{\tau=1}^t  \bbe_{(\bx_{\tau, i}, r_{\tau, i} ), i \in [n]} \left[ \left|f_2 \left( \bx_\tau^\ast ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \right]  \\
& \leq \underbrace{ \frac{1}{t}\sum_{\tau=1}^t \left|f_2 \left( \bx_\tau^\ast ; \widehat{\btheta}_{\tau-1}^2 \right) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right)  \right|}_{I_3}   + ( 1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}   ~.
\end{aligned}
\end{equation}


For $I_3$, according to Lemma \ref{lemma:caogeneli},  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$ , we have 
\begin{equation} 
\begin{aligned}
  & \frac{1}{t}\sum_{\tau=1}^t \left|  f_2 ( \bx_\tau^\ast ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right|   \\
   & \leq   \underbrace{ \frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau^\ast ; \widetilde{\btheta}^2 ) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right|}_{I_4}  + \calo \left( \frac{3L}{\sqrt{2t}} \right)~.
\end{aligned}
\end{equation}
 For $I_4$, according to  Lemma \ref{lemma:zhu} (1), these exists   $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0  \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, 
such that
\begin{equation} 
\begin{aligned}
 &\frac{1}{t} \sum_{\tau=1}^t \left|   f_2 ( \bx_\tau^\ast; \widetilde{\btheta}^2 ) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right|  \\
&\leq  \frac{1}{t} \sqrt{t} \sqrt{ \underbrace{ \sum_{\tau=1}^t \left(   f_2 ( \bx_\tau^\ast ; \widetilde{\btheta}^2 ) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2}_{I_5} } \\
&\leq  \frac{1}{\sqrt{t}}\sqrt{ \underbrace{2\epsilon}_{I_5}}~, 
\end{aligned}
\end{equation}
where $I_5$ follows by a direct application of  Lemma \ref{lemma:zhu} (1) by defining the loss $\mathcal{L}(\widetilde{\btheta}^2) =\frac{1}{2}\sum_{\tau=1}^t \left(   f_2 ( \bx_\tau^\ast ; \widetilde{\btheta}^2 ) - \left(r_\tau^\ast - f_1(\bx_\tau^\ast; \widehat{\btheta}_{\tau-1}^1) \right) \right)^2 \leq \epsilon$. 
Combining above inequalities, with probability $(1-3\delta)$ we have 
\begin{equation}\label{eq:fincon}
\begin{aligned}
 & \underset{(\bx_{t, i}, r_{t, i} ), i \in [n]}{\bbe}   \left[\left|f_2 \left( \bx_t^\ast ; \btheta_{t-1}^2\right) - \left(r_t^\ast - f_1(\bx_t^\ast; \btheta_{t-1}^1) \right)  \right| | \{ \bx_{\tau}, r_{\tau}\}_{\tau = 1}^{t-1} \right] \\
 & \qquad \leq   \sqrt{\frac{ 2\epsilon}{t}} +  \calo \left( \frac{3L}{\sqrt{2t}} \right)  + (1 + 2 \xi) \sqrt{ \frac{2 \log (1/\delta) }{t}}~.
 \end{aligned}
\end{equation}
Then, applying union bound to $t, n$ and rescaling the $\delta$ complete the proof.

\qed




%\abcomment{Have not explained why we need to take union bound over $t$, will be good to add that. Note that we have not maintianed the conditioning w.r.t.~the history $F_{\tau}$ through the proof, will also be good to do that.}












\begin{lemma} \label{lemma:a}
 
 Let $f(\cdot; \widehat{\btheta}_t)$ follow the stochastic gradient descent of $f_1$ or $f_2$ in Algorithm \ref{alg:main}.
 Suppose $m, \eta_1, \eta_2$ satisfy the conditions in Eq. (\ref{eq:condi}).  With probability at least $1 - \delta$, for any $\bx$ with $\|\bx\|_2 = 1$ and $t \in [T]$, it holds that
\[
| f(\bx; \widehat{\btheta}_t)| \leq  \mathcal{O}(1) +  \mathcal{O} \left( \frac{t^3n L \log m}{ \rho \sqrt{m} } \right) + \mathcal{O} \left(  \frac{t^4 n L^2  \log^{11/6} m}{ \rho^{4/3}  m^{1/6}}\right).
\]
\end{lemma}



%\begin{prove*}
\proof Considering an inequality $ |a - b| \leq c$, we have $|a| \leq |b| + c$. 
Let $\btheta_0$ be randomly initialized. Then applying  Lemma \ref{lemma:gu} (1),  for any $\bx \sim \mathcal{D}, \|\bx \|_2 = 1$ and $ \|\widehat{\btheta}_t - \btheta_0\| \leq w$,  we have 
\begin{equation}
\begin{aligned}
|f(\bx; \widehat{\btheta}_t) | &\leq  | f(\bx; \btheta_0)| +  |\langle  \triangledown_{\btheta_0}f(\bx_i; \btheta_0), \widehat{\btheta}_t - \btheta_0   \rangle  | +   \mathcal{O} ( L^2 \sqrt{m \log(m)}) \|\widehat{\btheta}_t - \btheta_0 \|_2 w^{1/3} \\
&  \leq \underbrace{\mathcal{O}(1)}_{I_0}  +  \underbrace{  \|  \triangledown_{\btheta_0}f(\bx_i; \btheta_0)  \|_2 \| \widehat{\btheta}_t - \btheta_0  \|_2}_{I_1}  + \mathcal{O} ( L^2 \sqrt{m \log(m)}) \|\widehat{\btheta}_t - \btheta_0 \|_2 w^{1/3} \\
& \leq \mathcal{O}(1) +  \underbrace{  \mathcal{O} (L) \cdot  \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)}_{I_2} + \underbrace{   \mathcal{O} \left( L^2 \sqrt{m \log(m)} \right) \cdot  \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)^{4/3} }_{I_3}  \\
&  =  \mathcal{O}(1) +  \mathcal{O} \left( \frac{t^3 L \log m}{ \rho \sqrt{m} } \right) + \mathcal{O} \left(  \frac{t^4 L^2  \log^{11/6} m}{ \rho^{4/3}  m^{1/6}}\right)
\end{aligned}
\end{equation}
where: $I_0$ is based on the Lemma \ref{lemma:zhu} (3);
$I_1$ is an application of Cauchy–Schwarz inequality; $I_2$ is according to  Lemma \ref{lemma:zhu} (2) and (3) in which $\widehat{\btheta}_t$ can be considered as one step gradient descent; $I_3$ is due to Lemma \ref{lemma:zhu} (2).

Then, the proof is completed. \qed
%\end{prove*}












\begin{lemma} \label{lemma:zhu}
Given a constant $0 < \epsilon < 1$, suppose $m \geq  \widetilde{\Omega}   \left ( \text{poly}(T, n, L, \rho^{-1}) \cdot    e^{\sqrt{\log 1/\delta }}  \right ) $, the learning rate $\eta = \Omega(\frac{\rho}{ \text{poly} (t ,n, L) m} ) $, the number of iterations $K = \Omega (\frac{\text{poly}(t, n, L)}{\rho^2} \cdot \log \epsilon^{-1})$. Then, with probability at least $1 - \delta$,  starting from random initialization $\btheta_0$, 
\begin{enumerate}[label=(\arabic*)]
    \item (Theorem 1 in \citep{allen2019convergence}) 
    In round $t \in [T]$, given the collected data $\{\bx_\tau, r_\tau\}_{i=\tau}^{t}$, the loss function is defined as:
    $\mathcal{L}(\btheta) = \frac{1}{2} \sum_{\tau = 1}^{t}   \left( f(\bx_{\tau}; \btheta) - r_\tau \right)^2$.
    Then,  there exists  $\widetilde{\btheta}$  satisfying $\|\widetilde{\btheta} - \btheta_0\|_2 \leq \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)$, such that
    $ \mathcal{L}(\widetilde{\btheta}) \leq \epsilon $ in $K = \Omega (\frac{\text{poly}(t, n, L)}{\rho^2} \cdot \log \epsilon^{-1})$ iterations;\\
    \item (Theorem 1 in \citep{allen2019convergence}) For any $k \in [K]$, it holds uniformly that
    $
    \|\btheta^{(k)}_t - \btheta_0\|_2 \leq \mathcal{O}\left( \frac{ t^3 }{\rho \sqrt{m}} \log m  \right)
    $;
    \item Following the initialization, it holds that
    \[
     \|   \triangledown_{\btheta_0 }f(\bx_i; \btheta_0)  \|_2 \leq \mathcal{O} (L),   \    \   \
      |  f(\bx_i; \btheta_0)  | \leq \mathcal{O} (1)
    \]
\end{enumerate}
where $\btheta^{(k)}_t$ represents the parameters of $f$ after $k \in [K] $ iterations if gradient descent in round $t$.
\end{lemma}

%\begin{prove*}
\proof 
Note that the output dimension $d$ in \citep{allen2019convergence} is removed because the output of network function in this paper always is a scalar.
For (1) and (2),  the only different setting from \citep{allen2019convergence} is that the initialization of last layer $\bw_{L} \sim \mathcal{N}(0, \frac{2}{m})$ in this paper while $\bw_{L} \sim \mathcal{N}(0, \frac{1}{d})$ in \citep{allen2019convergence}. Because $d =1$ and $m > d$ here, the upper bound in \citep{allen2019convergence} still holds for $\bw_L$: with probability at least $1 - \exp{(- \Omega(m/L))}, \|\bw_L\|_F \leq \sqrt{m/d}$. Therefore, it is easy to verify that (1) and (2) still hold for the initialization of this paper.

For (3), based on Lemma 7.1 in \cite{allen2019convergence}, we have $ |  f(\bx_i; \btheta_0)  | \leq \mathcal{O} (1)$. Denote by $D$ the ReLU function.  For any $l \in [L]$, 
\[
\|\triangledown_{W_l}f(\bx_i; \btheta_0)\|_F \leq   \|\bw_L D \bw_{L-1} \cdots D \bw_{l+1}\|_F \cdot \| D \bw_{l+1} \cdots \bx \|_F \leq  \mathcal{O}(\sqrt{L}) 
\] 
where the inequality is according to Lemma 7.2 in \cite{allen2019convergence}. Therefore, we have $ \|   \triangledown_{\btheta_0 }f(\bx_i; \btheta_0)  \|_2 \leq \mathcal{O} (L) $. \qed 
%\end{prove*}




\begin{lemma} [Lemma 4.1, \citep{cao2019generalization}]  \label{lemma:gu} 
Suppose $ \mathcal{O}( m^{-3/2} L^{-3/2} [ \log (TnL^2/\delta) ]^{3/2}  )   \leq w \leq  \mathcal{O} (L^{-6}[\log m]^{-3/2} )$. Then,
with probability at least $1- \delta$ over randomness of $\btheta_0$, for any $ t \in [T], \|\bx \|_2 =1 $, and $\btheta, \btheta'$
satisfying $\| \btheta - \btheta_0 \|_2 \leq w$ and $\| \btheta' - \btheta_0 \|_2 \leq w$
, it holds uniformly that
\begin{enumerate}[label=(\arabic*)]
 \item $
| f(\bx_i; \btheta) - f(\bx_i; \btheta') -  \langle  \triangledown_{\btheta'}f(\bx_i; \btheta'), \btheta - \btheta'    \rangle    | \leq \mathcal{O} (w^{1/3}L^2 \sqrt{m \log(m)}) \|\btheta - \btheta'\|_2
$
\item $  \| \triangledown_{\btheta}f(\bx; \btheta)\|_2  \leq \mathcal{O}(\sqrt{mL})$.
\end{enumerate}
\end{lemma}


\begin{lemma} \label{lemma:caogeneli}
For any $\delta > 0$, suppose
\[
m > \tilde{\mathcal{O}}\left(  \text{poly} (T, n, \rho^{-1}, L, \log (1/\delta) \cdot e^{\sqrt{ \log 1/\delta}}) \right).
\]
Then, with probability at least $1 - \delta$, setting $\eta_2 = \Theta( \frac{t^5}{ \delta^2 \sqrt{2}  m})$ for algorithm \ref{alg:main},   for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, it holds that
\[
\begin{aligned}
\sum_{\tau=1}^t \left|   f_2 \left( \frac{\triangledown_{\widehat{\btheta}_{\tau-1}^1 }f_1(\bx_\tau ; \widehat{\btheta}_{\tau-1}^1)}{c_1\sqrt{mL} } ; \widehat{\btheta}_{\tau-1}^2  \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| \\
\leq   \sum_{\tau=1}^t \left|   f_2  \left( \frac{\triangledown_{\widehat{\btheta}_{\tau-1}^1}f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1)}{c_1\sqrt{mL} } ; \widetilde{\btheta}^2 \right) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| + \calo \left(\frac{3L\sqrt{t} }{\sqrt{2}}\right) \\
\end{aligned}
\]
\end{lemma}
\begin{proof}
This is a direct application of Lemma 4.3 in \citep{cao2019generalization} by setting $R = \frac{t^3}{\rho} \log m,  \epsilon = \frac{LR}{ \sqrt{2\nu t}}$,  and $ \nu = \nu' R^2$, where $\nu'$ is some small enough absolute constant.
We set $L_\tau( \widehat{\btheta}_{\tau -1}^2 ) =  \left |  f_2 ( \triangledown_{\widehat{\btheta}_{\tau-1}^1} f_1  ; \widehat{\btheta}_{\tau-1}^2 ) - \left(r_\tau - f_1(\bx_\tau; \widehat{\btheta}_{\tau-1}^1) \right) \right| $.
Based on Lemma \ref{lemma:zhu} (2), for any $\tau \in [t]$, we have 
\[ 
\|\widehat{\btheta}_{\tau}^2 - \widehat{\btheta}_{\tau-1}^2\|_2 \leq  \| \widehat{\btheta}_{\tau}^2 - \btheta_0 \|_2 + \| \btheta_0 -   \widehat{\btheta}_{\tau-1}^2 \|_2 \leq \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m).
\]
Then, according to Lemma 4.3 in \citep{cao2019generalization}, then,  for any $\widetilde{\btheta}^2$ satisfying $\|   \widetilde{\btheta}^2  - \btheta^2_0    \|_2 \leq  \mathcal{O}(\frac{t^3}{\rho \sqrt{m} } \log m)$, there exist a small enough absolute constant $\nu'$,  such that 
\begin{equation}
\sum_{\tau=1}^t  L_\tau( \widehat{\btheta}_{\tau -1}^2 ) \leq \sum_{\tau=1}^t L_\tau( \widetilde{\btheta}^2) + 3 t \epsilon.
\end{equation}
Then, replacing $\epsilon$ completes the proof.
\end{proof}







==> analysis2.tex <==
\section{Comparison with Single Reward Function} \label{sec:the2p}

In this section, we provide the regret analysis of pure-exploitation approach, denoted by \sysn', i.e., the \sysn with $f_3 = f_1$.

\begin{theorem}
Let $f_1$ follow the setting of $f$ (Eq. (\ref{eq:structure}) ) and $f_3 = f_1$. Given one constant $\epsilon_1$,   $ 0 < \epsilon_1<1 $,  suppose
\begin{equation}\label{eq:condi}
\begin{aligned}
m &\geq \Omega( \text{poly} (T, n, L, \log (1/\delta) ) \cdot e^{\sqrt{ \log 1/\delta}}),  \  \  \eta_1   = \Theta  ( \frac{ \delta}{\text{poly}(T, n, L) \cdot m} );  \\
K_1  & = \Theta (\frac{ \text{poly}(T, n, L)  }{\delta^2} \cdot \log (\epsilon_1)^{-1}),  
\end{aligned}
\end{equation}
then with probability at least $1 - \delta$, the expected regret of \sysn' in $T$ rounds satisfies
\[
\mathbf{R}_T' \leq \mathcal{O} \left( (2\sqrt{T} -1)\sqrt{2 \epsilon_1} \right) +  \mathcal{O} \left( ( \xi_1 + 1) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} \right),
\]
where
\[
\xi_1 =  \mathcal{O} \left( \frac{T^4n L \log m}{ \delta \sqrt{m} } \right) + \mathcal{O} \left(  \frac{T^5 n L^2  \log^{11/6} m}{ \delta  m^{1/6}}\right) < 1 .
\]
When $\epsilon_1 \leq  1/T$, we have
\[
\mathbf{R}_T' \leq \mathcal{O} \left( 1 \right) +  \mathcal{O} \left( (\xi_1 + 1) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} \right).
\]
\label{theo2}
\end{theorem}


\para{Comparison with Theorem 1}. With the regret upper bounds of \sysn and \sysn', we have
\begin{equation}
\begin{aligned}
&\text{(\sysn)}  \ \  \mathbf{R}_T \leq \mathcal{O}(1) +    \mathcal{O} \left( (\xi_2 + \epsilon_1) (2 \sqrt{T} -1 ) \sqrt{2 \log ( \mathcal{O}(Tn)/\delta)}  \right) \\
&  \text{ (\sysn') }  \ \ 
\mathbf{R}_T' \leq \mathcal{O}(1) +    \mathcal{O} \left( (\xi_1 + 1) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}{(Tn)}/\delta)} \right) .
\end{aligned}
\end{equation}
Note that $\xi_1, \xi_2 < 1$ by setting of $m, m'$.  It is easy to observe that regret bound of \sysn is tighter than \sysn', because $\epsilon_1$ is a given number and can be $\epsilon_1 \ll 1$. Therefore, by adding a exploration network $f_2$,  \sysn can achieve a tighter bound than pure-exploitation approach.







%\begin{prove*}
{\em Proof of Theorem~\ref{theo2}.}
In round $t$, given the $n$ arms $(\bx_{t, 1}, \dots \bx_{t, n})$, let $ H_t =  ( h(\bx_{t, i}), \dots, h(\bx_{t, n})   )  $ denote their expected rewards. For brevity, for the selected arm $\bx_t$ in round $t$, let $h(\bx_t)$ be its expected reward and $\bx_t^\ast$ be the optimal arm in round $t$.

Then, based on the proof of Theorem \ref{theo1},  the expected regret of round $t$ is computed by
\[
\begin{aligned}
\mathbf{R}_t & = h(\bx_t^\ast) - h(\bx_t)  \\
&  \leq  h(\bx_t^\ast) - f_3(\bx_t^\ast)  +   f_3(\bx_t) - h(\bx_t) \\
&  \leq \max_{i \in [n]} \left( \bbe[ \left( f_3( r_{t, i} - \bx_{t, i})\right)  |  \bx_{t,i}] \right)  +     \bbe [ \left( f_3(\bx_t)  - r_t \right) | \bx_t ] \\
&  \leq      \max_{i \in [n]} \bbe [| f_1(\bx_{t, i}; \btheta^1_{t-1}) -  r_{t, i} | | \bx_{t,i} ]    +     \bbe [ |  f_1(\bx_i; \btheta^1_{t-1}) - r_t | | \bx_{t} ]
\end{aligned}
\]

Then, based on Lemma \ref{lemma:main2}, with probability at least $1-\delta$, we have
\[
\mathbf{R}_t  \leq  2 \left(
\sqrt{\frac{2 \epsilon_1 }{t}} + (\xi_1 +  1) \sqrt{ \frac{2 \log (\mathcal{O}(Tn)/\delta)}{t}} \right) 
\]

Then expected regret of $T$ rounds is computed by
\begin{equation}
\begin{aligned}
\mathbf{R}_T & = \sum_{t =1}^T \mathbf{R}_t\\
 & \leq 2 \sum_{t =1}^T   \left(
\sqrt{\frac{2 \epsilon_1}{t}} + (\xi_1 + 1) \sqrt{ \frac{2 \log (\mathcal{O}(Tn)/\delta)}{t}} \right)  \\
& < \underbrace{ 2 (2\sqrt{T} -1)\sqrt{2 \epsilon_1} + 2 (\xi_1 + 1) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)} }_{I_2}
\end{aligned}
\end{equation}
where  $I_2$ is because $\sum_{t=1}^T \frac{1}{\sqrt{t}}  \leq  \int_{1}^T   \frac{1}{\sqrt{t}}  \ dx  +1 =  2 \sqrt{T} -1$ \citep{chlebus2009approximate}.

When 
$K = \Omega (\frac{ \text{poly}(T, n, L)  }{\delta^2} \cdot \log T)$, according to Lemma 3.4,  with probability at least $1 - \delta$, we have $\epsilon_1 = 1/T$. Therefore, we have
\begin{equation}
\mathbf{R}_T \leq \mathcal{O}(1) +    2 (\xi_1 + 1) (2 \sqrt{T} -1 ) \sqrt{2 \log (\mathcal{O}(Tn)/\delta)}, 
\end{equation}
The proof is completed. \qed
%\end{prove*}



\begin{lemma} \label{lemma:main2}

Given $0< \epsilon_1 <1$, suppose $m, \eta $ satisfy the conditions in Eq. (\ref{eq:condi}) and $K_1 = \Omega (\frac{\text{poly}(T, n, L)}{\delta^2} \cdot \log \epsilon_1^{-1}) $. Then, with probability at least $1- \delta$, for any $t \in [T], i \in [n]$, it holds uniformly that
\[
\bbe_{(\bx_{t+1,i}, r_{t+1, i}) \sim \mathcal{D}} [  |r_{t+1,i} -  f_1(\bx_{t+1, i}; \btheta_t )|]  \leq   \sqrt{\frac{ 2 \epsilon_1 }{ t}} + (\xi_1  +1 )\sqrt{ \frac{ 2\log (\mathcal{O}(Tn)/\delta)}{t}} 
\]
\end{lemma}

%\begin{prove*}
\proof Applying Lemma \ref{lemma:a} on $f_1$, with probability at least $1- \delta$, for any $ t \in [T]$, it holds that $  |f_1(\bx; \theta_t)| \leq \xi_1$. And due to $ |r| \leq 1$ for any $(\bx, r) \sim \mathcal{D}$, we have 
\[
|r - f_1(\bx; \theta_t)| \leq \xi_1 + 1.
\]
Then, we have
\begin{equation}
 \frac{1}{t}\sum_{i=1}^t |r_i - f_1(\bx_i; \theta_t)|    \leq  \frac{1}{t} \sqrt{t}  \sqrt{ \sum_{i=1}^{t} (r_i - f_1(\bx_i; \theta_t))^2}   =    \underbrace{   \sqrt{ \frac{2 \mathcal{L}} {t} } \leq \sqrt{ \frac{2\epsilon_1}{t}} }_{I_1}.
\end{equation}
where $I_1$ is an application of Lemma \ref{lemma:zhu} (1). 


For any $i \in [t]$, given $(\bx_i, r_i) \sim \cald$, we 
set 
\[ V_{i} = \bbe_{(\bx_i, r_i) \sim D}[ | r_i - f_1(\bx_i; \btheta_t^1)   | ] - |r_i - f_1(\bx_i; \btheta_t^1)|.
\]

Then, we have
 \begin{equation} \label{eq:exp0}
 \begin{aligned}
 \bbe[  V_{i} | \mathbf{F}_i] = & \bbe_{(\bx_i, r_i) \sim D}\left[ \left| r_i - f_1(\bx_i; \btheta_t^1) \right| \right]   - \bbe \left[  \left|r_i - f_1(\bx_i; \btheta_t^1) \right| |  \mathbf{F}_i \right] = 0
\end{aligned}
 \end{equation}
where $ \mathbf{F}_i = (\bx_i, r_i)$ denotes the $\sigma$-algebra generated variables for $i \in [t]$.


And
\[
\begin{aligned}
\frac{1}{t} \sum_{i=1}^t  V_{i} = & \frac{1}{t}  \sum_{i=1}^t   \bbe_{(\bx_i, r_i) \sim D} \left[ \left|r_i - f_1(\bx_i; \btheta_t^1)  \right| \right]  \\
& - \frac{1}{t}  \sum_{i=1}^t \left|r_i - f_1(\bx_i; \btheta_t^1) \right| .
\end{aligned}
\] 






In the end, according to Lemma 1 in \citep{cesa2004generalization}, applying the Hoeffding-Azuma inequality to the bounded random variables $V_{1}, \dots, V_{t} $,  with probability at least $1 - \delta$,  we have 
\begin{equation}
\begin{aligned}
\bbe_{(\bx, r) \sim \cald} [|r - f_1(\bx; \btheta_t)|]  &=     \frac{1}{t} \sum_{i=1}^t  \bbe_{(\bx_i, r_i) \sim \cald} [ |r_i - f_1(\bx_i; \btheta_t)|  ]  \\
& \leq  \frac{1}{t}\sum_{i=1}^t |r_i - f_1(\bx_i; \theta_t)|   + (\xi_1 + 1) \sqrt{ \frac{2 \log (1/\delta) }{t}}\\
&  \leq  \sqrt{\frac{2 \epsilon_1 }{t}} + (\xi_1 + 1) \sqrt{ \frac{2 \log (1/\delta)}{t}} 
\end{aligned}
\end{equation}

Finally, rescaling $\delta$ completes the proof. \qed
%\end{prove*}










